SkillS: Adaptive Skill Sequencing for Efficient Temporally-Extended Exploration

The ability to effectively reuse prior knowledge is a key requirement when building general and flexible Reinforcement Learning (RL) agents. Skill reuse is one of the most common approaches, but current methods have considerable limitations.For example, fine-tuning an existing policy frequently fails, as the policy can degrade rapidly early in training. In a similar vein, distillation of expert behavior can lead to poor results when given sub-optimal experts. We compare several common approaches for skill transfer on multiple domains including changes in task and system dynamics. We identify how existing methods can fail and introduce an alternative approach to mitigate these problems. Our approach learns to sequence existing temporally-extended skills for exploration but learns the final policy directly from the raw experience. This conceptual split enables rapid adaptation and thus efficient data collection but without constraining the final solution.It significantly outperforms many classical methods across a suite of evaluation tasks and we use a broad set of ablations to highlight the importance of differentc omponents of our method.

==> S&T_arxiv2/abstract.tex <==
\begin{abstract}
The ability to effectively reuse prior knowledge is a key requirement when building general and flexible Reinforcement Learning (RL) agents. 
Skill reuse is one of the most common approaches, but current methods have considerable limitations.
For example, fine-tuning an existing policy frequently fails, as the policy can degrade rapidly early in training. %
In a similar vein, distillation of expert behavior can lead to poor results when given sub-optimal experts.
We compare several common approaches for skill transfer on multiple domains including changes in task and system dynamics. 
We identify how existing methods can fail and introduce an alternative approach to mitigate these problems. %
Our approach learns to sequence existing temporally-extended skills for exploration but learns the final policy directly from the raw experience. This conceptual split enables rapid adaptation and thus efficient data collection but without constraining the final solution. It significantly outperforms many classical methods across a suite of evaluation tasks and we use a broad set of ablations to highlight the importance of different components of our method.
\end{abstract}






==> S&T_arxiv2/background.tex <==
\section{Background}

We frame our discussion in terms of the reinforcement learning problem in which an agent observes the environment, takes an action, and receives a reward in response.
This can be formalized as a Markov Decision Process (MDP) consisting of the state space $\mathcal{S}$, the action space $\mathcal{A}$, and the transition probability $p(s_{t+1}|s_t,a_t)$ of reaching state $s_{t+1}$ from state $s_t$ when executing action $a_t$. 
The agent's behavior is given in terms of the policy $\pi(a_t | s_t)$.
In the following, the agent's policy $\pi$ can either be parametrised by a single neural network or further be composed of $N$ skills $\pi_i(a|s)$ such that $\pi(a|s) = f(a|\{\pi_i\}_{i=0..N-1}, s)$.

The agent aims to maximize the sum of discounted future rewards, denoted by:
\begin{equation}\label{eq:rl}
    J(\pi) = \mathbb{E}_{\rho_0\left(s_0\right),p(s_{t+1}|s_t,a_t),\pi(a_t|s_t)}\Big[\sum_{t=0}^{\infty} \gamma^{t} r_t \Big],
\end{equation}
where $\gamma$ is the discount factor, $r_t=r\left(s_{t}, a_{t}\right)$ is the reward and $\rho_0\left(s_0\right)$ is the initial state distribution. 
Given a policy we can define the state-action value function $Q(s_t, a_t)$ as the expected discounted return when taking an action $a_t$ in state $s_t$ and then following the policy $\pi$ as:
\begin{align} \label{eq:q_function}
    Q(s_t, a_t) &= r(s_t, a_t) + \gamma \E_{p(s_{t+1}|s_t, a_t), \pi(a|s_t)} [ Q(s_{t+1}, a) ].
\end{align}











==> S&T_arxiv2/backup/experiments.tex <==
\section{Experiments}
\label{experiments}

\subsection{Setup}
\label{experiments:setup}

The domains we consider for our experimental analysis can be broadly split into two categories: `Manipulation' and `Locomotion'. 

In the `Manipulation'  setting (see Figure \ref{fig:domains} (left)), a Sawyer robot arm equipped with Robotiq gripper
(for details on the setup, see Appendix \ref{appendix:skills}) is rewarded for bringing a set of three objects (green, yellow and blue) into a particular configuration. The configurations we consider include (in increasing order of complexity): `Lift' (lift the green object), `Stack' (stack green on yellow), `Pyramid` (stack green as a bridge on yellow and blue) and `Triple stack` (stack green on yellow and yellow on blue). As the task gets harder, we leverage previous task solutions as skills for the new setting. This is a natural transfer setting to test an agent's ability to build on previous knowledge and solve increasingly complex tasks. 
% For example, `Stack'  has access to the `Lift' skills while `Pyramid' has access to `Lift' and `Stack' skills.
For a full list of skills and tasks considered see Appendix \ref{appendix:experiment_details}).

For `Locomotion' (see Figure \ref{fig:domains} (right)), we consider a task where a bipedal OP3 robot \citep{} receives a sparse reward for scoring a goal with a wall blocking part of the path. Unlike in `Manipulation' where the transfer task changes, here we consider transferring to the same task but with different environment dynamics; a common problem faced when operating in the real world.

All the transfer tasks we consider use sparse rewards which are easier to define and are practically relevant for domains like robotics. We consider an off-policy distributed learning setup with a single actor and experience replay with full details provided in Appendix \ref{appendix:training_details}.

\begin{figure}
  \centering
    \includegraphics[width=\textwidth]{assets/images/domains.png}
\caption{\textbf{Domains:} The experimental domains used: (from left to right) `Manipulation' - Lift, Stack, Pyramid, Triple Stack and `Locomotion'- Goal-scoring. \label{fig:domains}}
\end{figure}

\subsection{How we analyse the performance}
Our method \met{} consists of two learning processes, one designed to quickly collect useful data (the scheduler) and one to distill the best solution for the task from the same data (the new skill). As our primary interest is in the task solution, unless otherwise specified, we report the \textit{performance of the new skill} when executed in isolation on the environment for the entire episode (see Fig. \ref{fig:skill_analysis}).
% The performance of the data collection could be instead analysed by looking at the reward collected by the Skill Scheduler itself (Fig. \ref{fig:scheduler_analysis}), see the Appendix for this further analysis. \giulia{Shall we keep it or not?} 
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.275\textwidth}
    \centering
  \includegraphics[width=\textwidth]{assets/images/new_skill_analysis_3.png}
  \vspace{1pt}
  \caption{\label{fig:skill_analysis}}
  \end{subfigure}
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
  \includegraphics[width=\textwidth]{assets/images/scheduler_analysis_2.png}
  \vspace{0.5pt}
   \caption{\label{fig:scheduler_analysis}}
  \end{subfigure}
     \hspace{4pt}
  \begin{subfigure}[b]{0.36\textwidth}
  \includegraphics[height=0.95cm, width=0.98\linewidth, trim=0 0 0 0, clip=true]{assets/figures/skill_execution_legend.png}
\includegraphics[width=\linewidth]{assets/figures/skill_execution.png}
\caption{\label{fig:skill_execution_plot}}
\end{subfigure}
\caption{\textbf{a) - b) Performance analysis} The new skill is evaluated by executing it in the environment for the entire episode (\ref{fig:skill_analysis}). This differs from the way the data is collected, as at training time the new skill can interact with the environment time only when selected by the scheduler (\ref{fig:scheduler_analysis}). \textbf{c) Skill execution:} The plot shows the consecutive execution of each skill, i.e. the number of timesteps each skill has been consecutively executed for. \giulia{replace plot}}
\end{figure}

\giulia{To update with total execution}
Before focusing on the new skill performance in the next sections, it is worth showing how the scheduler chooses the skills to interact with the environment.
In Fig. \ref{fig:skill_execution_plot} we show the skill selection during the training by plotting the average \textit{consecutive} execution for each skill. We assume 7 skills are available, some of them needed for solving the task at hand (`reach green', `close fingers'), while the others act as a distractor (e.g. `reach yellow' or `open fingers'). At the beginning the scheduler quickly selects the most useful skills (`reach green', `close fingers') while discarding those less relevant to the task (look at the drop in executing `reach yellow' or `reach blue'). Also, the scheduler does not initially choose the new skill as it performs poorly at the beginning of the training. Once the new skill improves (after roughly 200- episodes), the scheduler quickly understands to select it more often, becoming eventually the most executed skill.


\subsection{Analysis: Sparse locomotion and manipulation}
The goal of this section is to analyse how the different skill reuse methods perform when transferring to the domains defined in Section \ref{experiments:setup}. Figure \ref{fig:manipulation_sparse} shows the performance of skill-based approaches on the `Manipulation' domains \footnote{Given the sparse nature of the reward, note that most methods fail to learn at all and show up as flat lines in the plot.}. We observe that among all the methods that we considered only \met \ can learn effectively in these domains even though other methods have access to the same set of skills. Importantly this illustrates that reusing skills on its own is insufficient to guarantee good transfer performance. 

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{assets/figures/manipulation_sparse.png}
%   \caption{\textbf{Sparse Manipulation:} Performance of various skill transfer mechanisms on sparse manipulation tasks.}
%   \label{fig:manipulation_sparse}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sparse.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_sparse.png}
    \caption{Lifting}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sparse.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_sparse.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_sparse.png}
    \caption{Triple Stacking}
  \end{subfigure}
\caption{Performance of various skill transfer mechanisms on sparse-reward manipulation tasks. For each task, all approaches are given the previous, easier skills (see Appendix for details) to learn the new task.}
\label{fig:manipulation_sparse}
\end{figure}

TODO(dhruvat): Insert OP3 results here once ready.
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/op3_legend_goal_scoring.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/op3_goal_scoring.png}
  \end{subfigure}
\caption{Performance on sparse-reward locomotion task.}
\label{fig:op3_goal_scoring}
\end{figure}


\subsection{Ablations}
In this section we analyse \met \ to test its robustness and tease apart which of it's components are important and under what conditions. The key questions we seek to answer through our analysis are:
\begin{enumerate}
    \item How robust is \met \ to the number and quality of skills used?
    \item How does the analysis change when investing engineering effort to design dense rewards?
    \item Are there advantages to the flexibility of the infer mechanism? \dhruva{This feels a bit out of place here. Figure out structure once OP3 results are in.}
    \item Is the flexible temporal abstraction useful?
    \item How important is the temporally correlated exploration mechanism of \met?
    \item Does the separate inference mechanism provide any advantage?
    \giulia{Maybe point 2. and 6. can be merged together and we can analyse everything together?}
\end{enumerate}

\subsubsection{Robustness to number and type of skills}

Figure \ref{fig:ablation_num_skills} evaluates \met \ on the Stacking, Pyramid and Triple-stacking domains while changing the skill set $S$. For this analysis we vary the number of skills and the types of skills that the method has access to. In particular, we include a varying number of `distractor' skills that are not directly relevant for the task (e.g. reach `blue' for a task where `red' needs to be stacked, details in the Table \ref{tab:skills} in Appendix \ref{appendix:skills}). For the easier tasks of Stacking and Pyramid, the method is quite robust to various kinds of skills as long as there are \textit{some useful} skills in the set. When given only distractor skills, \met \ understandably fails to learn anything. On the most challenging task of Triple-stacking, increasing the number of skills has a detrimental effect of performance. We hypothesize that since more skills can greatly increase the size of the search space, it becomes much harder to randomly stumble onto the task solution. \dhruva{We could add a forward reference to the Discussion section here and discuss there ways to improve the method in future work to try to address this.}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{assets/figures/ablation_num_skills.png}
%   \caption{\textbf{Robustness to skills:} Performance when the number and type of skills changes.}
%   \label{fig:ablation_num_skills}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.5cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_skill_num.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_skill_num.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_skill_num.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_skill_num.png}
    \caption{Triple Stacking}
  \end{subfigure}
\caption{\textbf{Robustness to skills:} Performance when the number and type of skills changes.}
\label{fig:ablation_num_skills}
\end{figure}

\subsubsection{Performance with dense rewards.}

Figure \ref{fig:manipulation_staged} shows the performance with all skill transfer methods on the `Lift' and `Stacking' tasks when the agent has access to dense rewards. We observe that, in contrast to the sparse reward results of Figure \ref{fig:manipulation_sparse}, all methods learn effectively when provided with dense rewards. Since the reward provides a useful and reliable signal to guide learning there is less need to generate good exploration data using previous skills. The advantage of skill-based methods is thus primarily in domains where defining a dense reward is challenging but the required sub-behaviors are easier to specify.

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{assets/figures/manipulation_staged.png}
%   \caption{\textbf{Dense Manipulation:} Performance on dense manipulation tasks.}
%   \label{fig:manipulation_staged}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_dense.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_dense.png}
    \caption{Lifting}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_dense.png}
    \caption{Stacking}
  \end{subfigure}
\caption{Performance on dense-reward manipulation tasks. With carefully-tuned shaped rewards on simpler tasks, skill reuse is not as beneficial and all methods can learn effectively.}
\label{fig:manipulation_staged}
\end{figure}

\subsubsection{Flexibility of collect and infer}

% \begin{figure}
%   \centering
%   \includegraphics[height=6cm]{assets/figures/flexibility_c_i.png}
%   \caption{\textbf{Flexibility of collect and infer}}
%   \label{fig:ablation_separate_infer}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_flexibility.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_flexibility.png}
    \caption{Lifting}
    \label{fig:blocks_lift_flexibility}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_flexibility.png}
    \caption{Stacking}
    \label{fig:ablation_separate_infer}
  \end{subfigure}
\caption{Performance of \met~when combined with other approaches to transfer, showing its flexibility.}
\label{fig:manipulation_flexibility}
\end{figure}

\subsubsection{Flexible temporal abstraction}

Figure \ref{fig:ablation_temporal_abstraction} analyses the importance of the flexible temporal abstraction of \met. For this, we compare our method against a version dubbed `\met{} (fixed temporal abstraction)' where each skill, once chosen, is held fixed for a given duration (200 timesteps for episode of 600 timesteps). We observe that the performance on harder tasks (especially triple-stacking) degrades when using this constraint. Thus, the ability to flexibly choose the duration for which the skill is applied is quite important. \dhruva{We could make a point about options here and in the next ablation.}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.7\textwidth]{assets/figures/ablation_temporal_abstraction.png}
%   \caption{\textbf{Temporal abstraction:} Importance of flexible temporal abstraction.}
%   \label{fig:ablation_temporal_abstraction}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.5cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_flex_abs.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_flex_abs.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_flex_abs.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stack_flex_abs.png}
    \caption{Triple stacking}
  \end{subfigure}
\caption{\textbf{Temporal abstraction:} Importance of flexible temporal abstraction.}
\label{fig:ablation_temporal_abstraction}
\end{figure}

\subsubsection{Temporally correlated exploration}

Figure \ref{fig:ablation_temporal_correlation} illustrates the importance of temporally correlated exploration that arises from our formulation in Section \ref{method}. For this analysis we additionally run a version of our algorithm called `\met{} (without temporal abstraction)' where a new skill must be chosen at each timestep instead (i.e. $K=\{1\}$). In Figure \ref{fig:ablation_temporal_correlation} (left) we observe that, when given a single (near-)optimal skill\footnote{The near-optimal skill places the green object on the yellow one without moving the gripper away.}, all methods including regularisation and fine-tuning perform similarly. However, as shown in Figure \ref{fig:ablation_temporal_correlation} (right), when we use more than one sub-optimal skills temporally correlated exploration is crucial for learning.
 
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{assets/figures/ablation_temporal_correlation.png}
%   \caption{\textbf{Temporal correlation:} Importance of temporally correlated exploration.}
%   \label{fig:ablation_temporal_correlation}
% \end{figure}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
  \includegraphics[height=0.75cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_temporal2.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_single_temporal.png}
    \caption{Single optimal skill}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_multi_temporal.png}
    \caption{Multiple sub-optimal skills \label{fig:ablation_temporal_correlation}}
  \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[height=1cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sep_infer.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sep_infer.png}
    \caption{\label{fig:ablation_separate_infer}}
    \end{subfigure}
\caption{\textbf{a) - b) Temporal correlation:} Importance of temporally correlated exploration. \textbf{c) Separate infer:} Importance of having separate inference mechanism.}
\end{figure}

\subsubsection{Separate `infer' mechanism}
\label{separate_inference}

Finally, we conduct an experiment to study the importance of a separate `inference' (learning) mechanism as prescribed by the `Collect and Infer` paradigm. Figure \ref{fig:ablation_separate_infer}
compares the performance of \met{} (i.e. the inferred new skill when executed alone, as shown in Figure \ref{fig:skill_analysis}) against the performance of: `Scheduler' i.e. the Scheduler when executing the pre-trained skills $\mathrm{S}$ and the new skill (Figure \ref{fig:scheduler_analysis}), and `Scheduler (no new skill)', the performance of a Scheduler that can only execute the pre-trained fixed skills $\mathrm{S}$. As the figure shows, having a separate offline learning process is crucial for learning as the new skill (blue) outperforms the skill scheduler in performance, even when it can execute the new skill itself (light blue). The gap in performance is even more evident if the scheduler cannot access to the new skill (red).

% \begin{figure}
%   \centering
%   \includegraphics[height=6cm]{assets/figures/ablation_separate_infer.png}
%   \caption{\textbf{Separate infer:} Importance of having separate inference mechanism.}
%   \label{fig:ablation_separate_infer}
% \end{figure}
% \begin{figure}
% \begin{subfigure}[b]{0.5\textwidth}
% \includegraphics[height=1cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sep_infer.png}
% \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sep_infer.png}
% \caption{\textbf{Separate infer:} Importance of having separate inference mechanism.\label{fig:ablation_separate_infer}}
% \end{subfigure}
% \end{figure}

% What are our questions?
% \begin{itemize}
%     % \item Why is the scheduler so good? :) (placeholder)
%     \item How do different mechanisms for transfer relate to changes between source and target task? (what works well for dynamics vs reward changes)
%     \item How do different mechanisms for transfer relate to different task properties? (sparse v dense rewards)
%     \item How does temporal abstraction affect the performance for transfer?
%     \item How relevant is the distillation of behaviour into a single new policy? (and what makes it relevant)
% \end{itemize}

% The \met{} framework consists of two different learning processes with separate goals: 1) collecting data efficiently (the \method) and  2) inferring a task solution (the New Skill) that need to be evaluated separately.

% The way we evaluate the \method() and the New Policy is shown in Fig. \ref{fig:perf_eval}.
% \begin{itemize}
%     \item The \method{} is evaluated when executing the previously frozen skills and the New Policy. The desired behaviour consists of quickly collecting reward initially, while sub-optimal  performance at convergence are accepted\footnote{Sub-optimal performance at convergence is not a surprise as the \method does not have the same fine control as the New Policy, acting only at a larger time scale.}.
%     \item The New Policy is evaluated in isolation: it is executed for the entire episode. In this case, we want the final converged performance to be optimal as the New Policy is meant to provide the solution for the task.
% \end{itemize}

% In the next sections, we first analyse how the \method{} optimises the skill executions (Section \ref{skill_scheduler_analysis}) and then we analyse the quality of task solution we can obtain with the New Policy (Sections \ref{add section names}).
% \subsection{Skill scheduler vs baselines}

% \textit{How does our proposed method perform with respect to our transfer methods across different transfer scenarios (staged vs sparse reward), task changes vs dynamic changes?}

% \paragraph{Baselines}
% \begin{enumerate}
%     \item KL-reg
%     \item Skills reloading in RHPO
%     \item Fine-tuning (for OP3)
%     \item Dagger (Imitation learning)?
% \end{enumerate}

% \paragraph{Results}
% \begin{enumerate}
%     \item \textit{Sparse reward}. Skill scheduler outperforms all baselines
%     \begin{enumerate}
%     \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%             \item Stacking -> Pyramid
%             \item Stacking -> Triple stacking
%         \end{enumerate}
%      \item OP3 (transfer across dynamics or tasks?)
%         \begin{enumerate}
%             \item omni-directional walking -> 1v1?
%             \dhruva{Fine-tuning for omni-directional walking seems to fail even though reward is dense. We need to think about how to phrase this.}
%         \end{enumerate}
%     \end{enumerate}
% \end{enumerate}


% \begin{figure}
% \begin{center}
% \includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/images/blocks_legend_sparse.png}
% \end{center}
%   \centering
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{assets/images/blocks_lift_sparse.png}
%     \caption{Lifting}
%     \label{fig:blocks_lift_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_stack_sparse.png}
%     \caption{Stacking}
%     \label{fig:blocks_stack_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_pyramid_sparse.png}
%     \caption{Pyramid}
%     \label{fig:blocks_pyramid_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_triple_stacking_sparse.png}
%     \caption{Triple Stacking}
%     \label{fig:blocks_triple_sparse}
%   \end{subfigure}
% \caption{Transfer performance on four different manipulation tasks. For each task, all approaches are given the previous, easier skills (see Appendix for details) to learn the new task.}
% \end{figure}


% \subsection{Flexibility of separate Collect and Infer}
% \textit{Collect and infer gives great flexibility. What can we gain from it (i.e. using different methods for distilling the solution of the task)?}
% \subsubsection{Variations}
% \begin{enumerate}
%     \item Skill Scheduler vs
%     \item Skill Scheduler with KL-reg
%     \item Skill Scheduler with skills reloading in RHPO
% \end{enumerate}

% \subsubsection{Experiments}
% Maybe only with sparse reward here?
% \begin{enumerate}
%     \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%             \item Stacking -> Pyramid
%             \item Stacking -> Triple stacking
%             \dhruva{Perhaps here it is enough to include the hardest tasks?}
%         \end{enumerate}
%      \item OP3 (transfer across dynamics or tasks?)
%         \begin{enumerate}
%             \item omni-directional walking -> 1v1
%         \end{enumerate}
%     \end{enumerate}

% \subsection{Ablations on the Scheduler}
% \subsubsection{Dense versus sparse reward}
%  We show it is not so important with dense reward, everything works.
%     \begin{enumerate}
%         \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%         \end{enumerate}
%         \item OP3 (transfer across dynamics)
%         \begin{enumerate}
%             \item walk -> walk
%         \end{enumerate}
%     \end{enumerate}
    
%     \begin{figure}
% \begin{center}
% \includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/images/blocks_legend_sparse.png}
% \end{center}
%   \centering
%   \begin{subfigure}[b]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{assets/images/blocks_lift_dense.png}
%     \caption{Lifting}
%     \label{fig:blocks_lift_dense}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_stack_dense.png}
%     \caption{Stacking}
%     \label{fig:blocks_stack_dense}
%   \end{subfigure}
% \caption{Transfer performance on manipulation tasks with dense rewards. With carefully tuned, shaped rewards, skill reuse is not as beneficial and all methods can learn effectively.}
% \end{figure}

% \subsubsection{Impact of different number of skills}
% \textit{What is the impact of different number and quality of skills on our method?}
% Only in ablations add all transfer settings (i.e. different number of skills).

% \subsubsection{Importance of temporal correlated exploration}
% \textit{How important is temporally correlated exploration?}

% \subsubsection{Comparison}
% \begin{itemize}
%     \item Skill Scheduler vs
%     \item Skill Scheduler with learned skill length=1
% \end{itemize}

% \subsubsection{Tasks}
% \begin{itemize}
%     \item Stacking (multiple skills and single skill)
% \end{itemize}

% \subsubsection{Importance of temporal abstraction and flexible skill length}
% \textit{How important is temporal abstraction and flexible skill length?}
% \subsubsection{Comparison}
% \begin{itemize}
%     \item Skill Scheduler with fixed skill length (200)
%     \item Skill Scheduler with learned skill length (v/s Q-scheduler?)
% \end{itemize}

% \subsubsection{Tasks}
% \begin{itemize}
%     \item Stacking
%     \item Pyramid (we need at least until pyramid to see the real benefits)
%     \item Triple stacking?
% \end{itemize}


% \subsubsection{Importance of separate Infer process}
% \textit{What are the benefits of distilling the solution in a separate learning process?}

% We could compare New policy distilled with skill scheduler with modular RHPO with frozen skills or the skill scheduler without the new policy?

% Big plus 1, here we should also discuss the connection to the options framework \citep{sutton1999between} - describing the scheduled version as essentially a reparametrised version of options

==> S&T_arxiv2/backup/intro_paragraph.tex <==
With \method~(\met), we develop a method to satisfy these desiderata. We focus on the transfer of skills via their generated experience inspired by the Collect \& Infer perspective~\citep{riedmiller2022collect_infer, Riedmiller2018sacx}. Our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration via fast composition, but allows the final solution to deviate from the prior skills. 
% ### MERGE
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained off-policy with the same objective. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.
% This can also be interpreted via the lens of fast and slow learning: the scheduler can quickly learn to compose existing temporally-abstract skills and reach a coarse solution, while the new policy can more slowly infer an optimal solution from the gathered data.
With these components, the desiderata are split into easier-to-solve subgroups.
% ### MERGE


Current versions/parts:

Nicolas
With \method~(\met), we develop a method to satisfy these desiderata. Inspired by the Collect \& Infer paradigm~\citep{riedmiller2022collect_infer},our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration and fast adaptation, but allows the final solution to deviate from the prior skills.
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we also refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, thus incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained via off-policy RL also to maximize the task reward. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.

Dushyant
... our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration, but allows the final solution to deviate from the prior skills.
This can also be interpreted via the lens of fast and slow learning: the scheduler can quickly learn to compose existing temporally-abstract skills and reach a coarse solution, while the new policy can more slowly infer an optimal solution from the gathered data.

Giulia
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we also refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, thus incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained via off-policy RL also to maximize the task reward. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.


==> S&T_arxiv2/backup/method.tex <==
\section{Method}
\label{method}
% - The method{} we propose reuses skills -> skill assumptions
% - The method{} we propose is based on Collect and Infer
% - High level description of all the pieces
% - Scheduler and HCMPO
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{assets/images/SkillS_newskill.png}
    \caption{\textbf{The \met{} framework.} The data collection is performed by the Scheduler, a high level policy that chooses the best skills to execute among a set of pre-trained and frozen skills and the New Skill. The data collected via the interaction of all the skills and the environment is used to improve the Scheduler and the New Skill in two learning processes, using respectively the algorithms Hierarchical Categorical MPO (see Section \ref{hcmpo}) and Critic Regulatirized Regression (CRR, \cite{wang2020critic}.}
    \label{fig:SkillS}
\end{figure}

% The method we propose in this paper, named \textit{\met}, exploits a set $\mathrm{S}$ of $N$ previously trained skills
% \begin{equation}
%     \mathrm{S} = \{\pi_i(a|s)\}_{i=0}^{N-1}
% \end{equation}
% to bootstrap data collection for learning challenging sparse reward tasks.

The method we propose in this paper, named \textit{\met}, is based on the Collect and Infer framework, which assumes that data collection and inference of the solution are carried out in two separate processes (Fig. \ref{fig:SkillS}). The data collection is performed by the \textit{Scheduler}, a high level policy that chooses the best skills to execute in the environment in order to gather interaction data. The inference process consists of an off-policy learning algorithm that optimizes a \textit{New Skill} $\pi_{N}(a|s, \phi)$ for the task at hand.%In particular our method consists of the \textit{\method{}} or \textit{Collector} that collects data using a set of  skills $\mathrm{S}$ and a \textit{New Skill} $\pi_{N, \phi}(a|s)$ that infers the task solution from this data.



\subsection{Scheduler}
The \textit{Scheduler} is represented by a categorical policy
\begin{equation}
    \pi_{S}(z = [i; k]|s, \theta)
\end{equation} that outputs an action $z$ consisting of:
\begin{itemize}
    \item the index $i \in [0, .., N]$ of the skill to execute among $N$ previously trained and frozen skills $\mathrm{S}$:
    \begin{equation}
        \mathrm{S} = \{\pi_i(a|s)\}_{i=0}^{N-1}  \text{ where } |\bar{\mathrm{S}}|= N,
    \end{equation}
    and the \textit{New Skill}:
    \begin{equation}
        \bar{\mathrm{S}} = \mathrm{S} \cup \{\pi_{N}(a|s, \phi)\} \text{ where } |\bar{\mathrm{S}}|= N + 1,
    \end{equation}
        \item and the number of steps the skill is executed for $k \in \mathrm{K}$ (the \textit{skill length}), where $\mathrm{K}$ is a set of available skill lengths (positive integers) with cardinality $|\mathrm{K}| = M$.
\end{itemize}

Whenever a new action $z = [i; k]$ is chosen by the \method{}, the skill $\pi_{i}(a|s)$ (or $\pi_{N}(a|s, \phi)$ if $i=N$) is executed in the environment for $k$ time steps.
The scheduler does not sample any new action until the current skill length $k$ is expired (see Fig. \ref{fig:action_and_counter}). %If none of the available skill lengths $k \in \mathrm{K}$ is 1, this means the scheduler chooses a new skill at a larger time scale than the time scale at which the skills interact with the environment. 
Choosing $k>1$ means that the scheduler selects a new skill at a time scale that is different from the one at which the agent interacts with the environment. This induces temporal correlations in the agent's action choices which are important for skill-based exploration to be successful in sparse-reward tasks (see Section \ref{experiments}).
%This enforces a \textit{temporally correlated exploration} that is crucial for solving challenging sparse reward tasks, as shown in Section \ref{experiments}. 

Choosing the skill duration up-front introduces a nonstationarity in the agent's behavior. 
%In order to take into account for the flexible time scale during training 
To be able to frame the learning problem as an MDP we make use of an auxiliary variable $c$ named \textit{counter}. Whenever the scheduler chooses a new action $z = [i; k]$ the counter is set equal to chosen skill duration $c = k$. It is then decreased at every time step ($c_{t+1} = c_t - 1$) until the chosen skill duration has been reached and %skill length expires and 
the scheduler chooses a new action (see Fig. \ref{fig:action_and_counter}). The counter is crucial for learning of the critic, as is shown in Section \ref{hcmpo}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{assets/images/action_and_counter_new.png}
    \caption{\textbf{Scheduler action sampling and counter value generation.} This figure explains through an example how the \method{} interacts with the environment. At time $t=0$ the Scheduler samples an action $z_0=[i_0; k_0]$. This means that the low-level actions sampled from the same skill with index $i_0 \in \bar{\mathrm{S}}$ are applied  on the environment for $k_0$ time steps (e.g. $a_t \sim \pi_{i_0}(a|s_t)$ for $t=0, \dots, k_0 -1$, with $k_0 = 10$ in the figure). The scheduler does not sample any new action $z = [i; k]$ until the skill length $k_0$ has expired, i.e. when $t=k_0=10$. The counter is reset to be equal to the new chosen skill length $c_t = k_t$ every time a new scheduler action $z_t = [i_t; k_t]$ is sampled and is decreased every time step.}
    \label{fig:action_and_counter}
\end{figure}


The data collected by the \method{} is in the form $(s, a, z, c, r)$ and is used both to train the scheduler to improve the data collection and the New Skill to solve the task. In particular, the \method{} is trained only using the high-level actions, i.e. $(s, \mathbf{z}, c, r)$. While many objectives could be used to optimize the scheduler for data collection, in this work we decide to use the accumulated task return over the episode with duration $T$, $\sum_{t=0}^{T}\gamma^t r_t.$



We propose a novel algorithm to train the \method{} named \textit{Hierarchical Categorical MPO} (HCMPO) that takes into account the flexible time scale at which the scheduler chooses new actions. More details are provided in Section \ref{hcmpo}.

\subsection{The New Skill}
The New Skill $\pi_{N}(a|s, \phi)$ interacts with the environment only when chosen by the Skill Scheduler. It is trained with the data $(s, a, r)$\footnote{The New Skill is trained using the low-level actions $a$ as it is required to output actions compatible with the environment. Note also that the counter $c$ is not used for training the New Skill.} collected by the frozen skills $\mathrm{S}$ and the New Skill itself according to the scheduler decisions. Given the strongly off-policy nature of this data\footnote{At the beginning of the training the New Skill is not executed often as it is less likely to provide reward signal than the other skills.}, we train  the New Skill via Critic Regularized Regression \citep{wang2020critic} using  the accumulated task reward $\sum_{t=0}^{T}\gamma^t r_t$ as training objective, like for the Scheduler.

Note that, although the \method{} and the New Skill are trained with the same objective, we consider the New Skill to provide the final solution for the task at hand, as it can reach higher performance being distilled \textit{from scratch} on the collected data. The Scheduler is instead more suited to quickly collect data by design: having access to pre-trained skills facilitates exploration but can lead to sub-optimal performance in the limit as it constraints the final behaviour.



\subsection{Hierarchical Categorical MPO} \label{hcmpo} 
The framework we propose in this work differs from existing work~\citep{Heess2016locomotioncontroller,Wulfmeier2020rhpo} as 1) the high-level controller (the Scheduler) and the \textit{new} low-level controller (the New Skill)\footnote{The other skills $\mathrm{S}$ are kept frozen and not trained.} are trained in two separate learning processes and 2) the high-level controller is trained taking into account the flexible time scale at which the high-level actions are chosen~\citep{??}. In this section we explain the algorithm Hierarchical Categorical MPO (HCMPO) we use for training the high-level controller, i.e. the \method{}.

HCMPO builds on top of MPO with discrete action space ~\citep{neunert2020continuous} modifying the way the Policy Evaluation (PE) and Improvement (PI) are executed.

\textbf{Policy Evaluation (PE).}
In order to derive the PE updates we write down the probability that the scheduler chooses an action $z_t$ and the relative counter $c_t$:
\begin{align}
  \label{action_prob}
  \pi(z_t, c_t | s_t, z_{t-1}, c_{t-1}) &= \nonumber \\
  \pi(i_t, k_t, c_t | s_t, i_{t-1}, k_{t-1}, c_{t-1}) &=
  \begin{cases}
    \pi_{S}(z_t = [i_t; k_t]|s_t, \theta)\delta(k_t, c_t)  \text{ if } c_{t-1} = 1 \\
  \delta(i_t - i_{t-1})\delta(k_t - k_{t-1})\delta(c_t - (c_{t-1} - 1)) \text{ otherwise.}
  \end{cases}
\end{align}


This takes into account the fact that, if $k_{t}$ time steps have passed, i.e. the counter $c_{t}$ has expired, the scheduler chooses a new action $z_t=[i_t; k_t]$ at time $t$. It keeps the previous action  $z_t=z_{t-1}=[i_{t-1}; k_{t-1}]$ otherwise.

We can now use \eqref{action_prob} to derive the PE update rules:
\begin{equation}
  \label{policy_eval}
    Q(s_t, c_t, i_t, k_t)& \xleftarrow{} r_t +  \gamma \begin{cases}
    E_{\pi_{S}(i;k|s_{t+1})}[Q(s_{t+1}, c_{t+1}, i, k, \theta)] \text{ if } c_{t+1}= 1 \\
    Q(s_{t+1}, c_{t+1} = c_t - 1, i_{t+1}  = i_t, k_{t+1} = k_t) \text{ otherwise.}\\
\end{cases}
\end{equation}
If in the state $s_{t+1}$ the Scheduler has chosen a new action, the critic in state $s_t$ is updated with the standard MPO policy evaluation, i.e. with the critic evaluated using actions sampled from the current Scheduler policy in the next state $i, k \sim \pi_{S, \theta}(i;k|s_{t+1})$. In all the other states instead, the critic is updated with the critic computed using the action $z_{t+1}$ actually taken by the Scheduler, which is $z_{t+1} =  z_t = [i_t; k_t]$.

\textbf{Policy Improvement}
The Scheduler policy is improved following the MPO PI mechanism but only using the state-action pairs that correspond to a new action sampled by the Scheduler:
\begin{align}
   \label{policy_impr}
    \pi_{S}^{n+1} = \arg \max_{\pi_{S}} \sum_j  \sum_h q_{h,j} & \log(\pi_{S}(i_h, k_h | s_j, \theta))\\
    q_{h,j} = \frac{\exp{Q^{\pi_{S}^{n}}(s_j, c_j = 1, i, k)}}{ \sum_i{\exp{Q^{\pi_{S}^{n}}(s_j, c_j = 1, i, k)}}},
\end{align}
where $n$ is the index for the learning updates, $j$ and $h$  the indices that takes into account respectively the sampled states and actions.

\subsection{Data Augmentation}
Equations \eqref{policy_eval} and \eqref{policy_impr} show that only a subset of the available data $(s, z, c, r)$ is actively used for learning the scheduler critic and policy, i.e. only those states $s$ where the scheduler chooses a new action $z = [i; k]$. This effect is even stronger if the skill lengths $k \in \mathrm{K}$ are $>> 1$, as a new scheduler action $z$ is sampled less frequently. While large skill lengths induce temporal correlations that are important for skill-based exploration, it has the side effect of decreasing the data actively contributing to improve the scheduler. In order to maximize sample efficiency without sacrificing exploration, we augment the data as described in the appendix.%as follows.

\markus{Recommended split for the appendix part here. This also includes moving the corresponding figure.}

We define a \textit{skill trajectory} $\tau$ as the sequence of  $k^*$ time steps where the same skill with index $i^*$ is executed:
\begin{equation}
    \tau = \{(s_t, z_t=[i^*, k^*], c_t, r_t)\}_{t=t_0}^{t=t_0 + k^* - 1}
\end{equation}
and $k_{min}$ the smallest skill length available to the scheduler ($k_{min} \leq k $ for $k \in \mathrm{K}$ and $k_{min} \in \mathrm{K}$ ).

For every trajectory $\tau$ with skill length $k^*$ that can be written as multiple of the minimum skill length $k_{min}$ ($ mod(k_t, k_{min}) = 0$), we generate a new \textit{duplicated skill trajectory} $\bar{\tau}$ pretending it was generated by a scheduler choosing the same skill $i^*$ multiple times with the smallest available skill length $k_{min}$ (see Fig. \ref{fig:data_augmentation}).  This generates a new trajectory that is compatible with the data actually collected, as the skill $i^*$ is executed for $k^*$ consecutive time steps also in $\bar{\tau}$. However, the new trajectory has more samples that are actively used for improving the scheduler and the policy, as it pretends the scheduler made a decision in more states. Both $\tau$ and $\bar{\tau}$ are added to the replay and used for training the scheduler. Technical details on the data augmentation are provided in Appendix \ref{appendix:data_aug}.



\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/images/data_augmentation.png}
    \caption{\textbf{Example of data augmentation.} Let's assume we have a trajectory $\tau$ where the skill with index $i^*$ is executed for $k^* = 60$ time steps. The duplicated trajectory $\bar{\tau}$ is generated by pretending the scheduler chose the same skill with index $i^*$ every $k_{min}$ time steps, equal to 10 in our example. This generates a new trajectory $\bar{\tau}$ compatible with the low-level actions $a_t$ and state $s_t$ actually collected during the interaction with the environment. }
    \label{fig:data_augmentation}
\end{figure}



\markus{To add: This perspective is highly related to efficiently learning high-level controllers over sets of options in the context of intra-option learning (using data throughout option execution to train the inter option policy) \citep{sutton1999between}.}

==> S&T_arxiv2/conclusions.tex <==





==> S&T_arxiv2/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Transferring the knowledge of reinforcement learning agents via skills or policies has been a long-standing challenge. Here, we investigate different types of task and dynamics variations and introduce a new method, \met, that learns using data generated by sequencing skills.
This approach demonstrates strong performance in challenging simulated robot manipulation and locomotion tasks. It further overcomes limitations of fine-tuning, imitation and purely hierarchical approaches. It achieves this by explicitly using two learning processes. The high-level scheduler can learn to sequence temporally-extended skills and bias exploration towards useful regions of trajectory space, and the new skill can then learn an optimal task solution off-policy. 




There are a number of interesting directions for future work. For instance, unlike in the options framework \citep{sutton1999between} which associates a termination condition with each option, in our work the duration of execution of a skill is independent of the pretrained skill. While this provides more flexibility during transfer, it also ignores prior knowledge of the domain, which may be preferable in some settings. Similarly, the high-level controller is currently trained to maximize task reward. However, it may be desirable to optimize the scheduler with respect to an objective that incentivizes exploration, e.g. to reduce uncertainty with regards to the value or system dynamics, improving its ability to collect data in harder exploration problems. Finally, our approach can naturally be combined with transfer of forms of prior knowledge apart from skills, such as prior experience data, the value function \citep{galashov2020IWPA}, or a dynamics model \citep{byravan2021evaluating} and we expect this to provide fertile area of future research.


==> S&T_arxiv2/experiments2.tex <==
\section{Experiments}
\label{experiments}

\begin{figure}
  \centering
    \includegraphics[width=0.8\textwidth]{assets/images/domains.png}
\caption{\textbf{Domains:} The experimental domains used: (from left to right) manipulation - Lift, Stack, Pyramid, Triple Stack and locomotion - GoalScoring and GetUpAndWalk. \label{fig:domains}}
\end{figure}

\paragraph{Environments}
We empirically evaluate our method in robotic manipulation and locomotion domains. The goal of our evaluation is to study how different skill transfer mechanisms fare in new tasks which require skill reuse.
In the manipulation setting (Fig. \ref{fig:domains} (left)), we utilise a simulated Sawyer robot arm equipped with Robotiq gripper and a set of three objects (green, yellow and blue)~\citep{Wulfmeier2020rhpo}. We consider four tasks of increasing complexity: Lift the green object, Stack green on yellow, building a Pyramid of green on yellow and blue, and Triple stack with green on yellow and yellow on blue. Every harder task leverages previous task solutions as skills: this is a natural transfer setting to test an agent's ability to build on previous knowledge and solve increasingly complex tasks.
For locomotion (Fig. \ref{fig:domains} (right)), we consider two tasks with a simulated version of the OP3 humanoid robot~\citep{robotisOP3}: GetUpAndWalk and GoalScoring. The GetUpAndWalk task requires the robot to compose two skills: one to get up off of the floor and one to walk. In the GoalScoring task, the robot gets a sparse reward for scoring a goal, with a wall as an obstacle. The GoalScoring task uses a single skill but is transferred to a setting with different environment dynamics. This allows us to extend the study beyond skill composition to skill adaptability; both of which are important requirements when operating in the real world.
All the considered transfer tasks use sparse rewards\footnote{When the reward provides a reliable learning signal (e.g. in case of dense rewards) there is less need to generate good exploration data using previous skills. The advantage of skill-based methods is thus primarily in domains where defining a dense, easier-to-optimise reward is challenging.  %
For more details see Appendix \ref{appendix:dense_rewards}.} except the GetUpAndWalk task where a dense walking reward is given but only if the robot is standing. 
We consider an off-policy distributed learning setup with a single actor and experience replay. \rebuttal{For each setting we plot the mean performance averaged across 5 seeds with the shaded region representing one standard deviation.}
More details on the skills and tasks can be found in Appendix \ref{appendix:experiment_details}.
\paragraph{Analysis details}
Our method \met{} consists of two learning processes, one designed to quickly collect useful data (the scheduler) and one to distill the best solution for the task from the same data (the new skill). As our primary interest is in the task solution, unless otherwise specified, we focus on the \textit{performance of the new skill} when executed in the environment in isolation for the entire episode. See Appendix \ref{appendix:performance_analysis} for details about how the new skill and the scheduler can be separately evaluated.
We compare \met{} against the following skill reuse methods: Fine-tuning, RHPO, KL-regularisation (KL-reg. to Mixture) and DAGGER. Hierarchical RL via RHPO \citep{Wulfmeier2020rhpo} trains Gaussian mixture policies, and we adapt this method to reload skills as the components of the mixture. We can then either freeze the skills and include a new learned component (RHPO) or continue training the reloaded skills (fine-tuning). KL-reg. to Mixture adapts the MPO algorithm \citep{abdolmaleki2018maximum} to include a regularisation objective to distill the reloaded skills; and DAGGER adapts \cite{ross2011reduction} for imitation learning with previous skills. A full description of our baseline methods can be found in Appendix \ref{appendix:baseline_details}.

\subsection{Analysis: Sparse Reward Tasks in Locomotion and Manipulation}
Fig. \ref{fig:manipulation_sparse} shows the performance of skill-based approaches on manipulation domains\footnote{Given the sparse nature of the reward, most methods fail to learn at all and appear as flat lines in the plot.}. We observe that among all the considered methods, only \met \ can learn effectively in these domains, even though other methods have access to the same set of skills. %
When given access to a Lift task, all baselines still struggle to learn how to Stack. In contrast, \met{} can even learn challenging tasks like TripleStack with enough data. Importantly this illustrates that skill reuse on its own is insufficient to guarantee effective transfer, and highlights the strong benefit of temporal abstraction. While other methods such as RHPO switch between skills at high frequency, the scheduler's action space encourages the execution of skills over longer horizons, considerably reducing the search space.

Fig. \ref{fig:op3}a-b compares performance in the locomotion setting. In the GetUpAndWalk task, we find \met \  outperforms the other methods, confirming that temporal abstraction is fundamental when solving tasks that require %
a sequence of skills to be learned (getting up and then walking in this task). Executing the skills for longer horizons also generates higher reward early during training. Particularly poor is the performance of regularising towards a mixture of these skills as it performs worse than learning from scratch.
For the GoalScoring task which requires transferring a single skill to new dynamics, \met \ is competitive and shares the strongest results. As we will demonstrate in Section \ref{sec:temporal_abstraction}, the advantage of temporally correlated exploration conferred by \met \ is less important in settings with only one skill.

\begin{figure}
\centering
\includegraphics[height=0.5cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sparse.png}
  \centering
  \begin{subfigure}[b]{0.245\textwidth}
    \centering
    \includegraphics[width=\textwidth,]{assets/figures/blocks_lift_sparse.png}
    \vspace{-1.5em}
    \caption{Lift}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.245\textwidth}
    \centering
    \includegraphics[width=\linewidth,]{assets/figures/blocks_stack_sparse.png}
    \vspace{-1.5em}
    \caption{Stack}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.245\textwidth}
    \centering
    \includegraphics[width=\linewidth,]{assets/figures/blocks_pyramid_sparse.png}
    \vspace{-1.5em}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.245\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_sparse.png}
    \vspace{-1.5em}
    \caption{Triple Stacking}
  \end{subfigure}
 \vspace{-1.5em}
\caption{Performance of various skill transfer mechanisms on sparse-reward manipulation tasks. For each task, all approaches are given the previously trained useful skills (see Appendix for details) to learn the new task. \met{} is the only method to consistently learn across all tasks.}
\label{fig:manipulation_sparse}
\end{figure}



\begin{figure}
\includegraphics[height=0.7cm, trim=0 0 0 0, clip=true]{assets/figures/locomotion_sparse_legend.png}
 \includegraphics[height=0.75cm, trim=0 0 0 0, clip=true]{assets/figures/skill_execution_legend.png}
\begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=\linewidth]{assets/figures/op3_getup_walk.png}
\caption{GetUpAndWalk}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=\linewidth]{assets/figures/op3_goal_scoring.png}
\caption{GoalScoring}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.31\textwidth}
\includegraphics[width=\linewidth]{assets/figures/skill_execution.png}
  \caption{Skill execution. \label{fig:skill_execution_plot}}
  \end{subfigure}
\caption{(a) - (b) Performance on skill transfer methods on locomotion tasks. \met{} outperforms other methods in GetUpAndWalk (a) and
is no worse than other methods in the single skill GoalScoring task (b). (c) Skill average execution (as number of timesteps) during training.
\label{fig:op3}}
\end{figure}





\subsection{Ablations}
In this section we analyse the robustness of \met \ and evaluate the importance of various components and design decisions. In particular, we analyse (1) the scheduler skill selection during training; (2) the robustness to the number and quality of skills used; (3) the benefit and flexibility of having a separate infer mechanism and (4) the utility of flexible temporal abstraction. More ablations including a study of dense and sparse rewards, the benefit of offline methods like CRR and the importance of data augmentation can be found in Appendix \ref{appendix: additional}.

\subsubsection{Scheduler Skill Selection%
}
In this section we show how the scheduler typically chooses the skills to interact with the environment.
Fig. \ref{fig:skill_execution_plot} displays the skill selection during the training by means of the average \textit{consecutive} execution for each skill. We assume 7 skills are available, some of them needed for solving the task at hand (`reach green', `close fingers'), while the others act as a distractor (e.g. `reach yellow' or `open fingers'). At the beginning the scheduler quickly selects the most useful skills (`reach green', `close fingers') while discarding those less relevant to the task (observe the drop in executing `reach yellow' or `reach blue'). While the scheduler does not choose the poorly performing new skill early in training, eventually (after roughly 2000 episodes) it is selected more often until finally it is the most executed skill.

\subsubsection{Robustness to Skill Number and Quality}

Fig. \ref{fig:ablation_num_skills} evaluates \met \ on the stacking, pyramid and triple-stacking domains while changing the skill set $S$. For this analysis we vary the number\rebuttal{\footnote{\rebuttal{In order to augment the number of skills, we use 3 skills trained to solve the same task (e.g. `reach blue')  from different seeds and we refer to these sets in Fig. \ref{fig:ablation_num_skills}  as \textit{many distractors} and \textit{many useful skills}}.}} and the types of skills by including a variety of \textit{distractor} skills not directly relevant for the task (e.g. `reach blue' when `red' needs to be stacked; more details in Appendix \ref{appendix:skills}). With only distractor skills, \met \ understandably fails to learn anything. For the easier tasks of Stacking and Pyramid, \met \ is quite robust as long as there are \textit{some useful} skills in the set $S$. On the challenging triple-stacking task, increasing the number of skills has a detrimental effect on performance. We hypothesize that the larger skill set increases the size of the search space to a point where the exploration in skill space does not easily find the task solution.

\begin{figure}
\centering
\includegraphics[height=0.45cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_skill_num.png}

  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_skill_num.png}
    \vspace{-1.5em}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_skill_num.png}
    \vspace{-1.5em}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_skill_num.png}
    \vspace{-1.5em}
    \caption{Triple Stacking}
  \end{subfigure}
 \vspace{-0.5em}
\caption{\met{} can learn even when the number and type of skills change although performance deteriorates on harder tasks.}
\label{fig:ablation_num_skills}
\end{figure}


\subsubsection{Benefit of Separate Collect and Infer Mechanisms}
\label{separate_inference}

We conduct an experiment to study the importance of a separate \textit{inference} (learning) mechanism in extension of the hierarchical agent - the scheduler. %
Fig. \ref{fig:ablation_separate_infer} \rebuttal{compares the performance of the two components of \met{}: `Scheduler (incl. new skill)' which has access to the new skill and frozen skills and `New skill' which is the inferred new skill. In addition, we include a version `Scheduler (without new skill)' where the higher level scheduler \textit{only} has access to the frozen skills. }
As the figure shows, having a separate off-policy learning process is crucial for learning as the new skill (blue) outperforms the scheduler in performance, even when it can execute the new skill itself (red). The gap in performance is even more evident if the scheduler cannot access the new skill (light blue). 


\begin{figure}
\centering
\begin{subfigure}[b]{0.31\textwidth}
\centering
   \includegraphics[height=1cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sep_infer.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sep_infer.png}
    \captionof{figure}{Benefit of collect and infer. \label{fig:ablation_separate_infer}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.31\textwidth}
  \centering
  \includegraphics[height=0.75cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_temporal.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_single_temporal.png}
    \caption{Single optimal skill. \label{fig:single-skill}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_multi_temporal.png}
    \caption{Multiple sub-optimal skills. \label{fig:multiple-skill}}
\end{subfigure}
\caption{(a) \met{} performs best when given access to a separately inferred new skill.
(b)-(c) The main advantage of \met{} is likely due to temporally correlated exploration. When given access to a single optimal skill (b) all methods can learn effectively but with multiple sub-optimal skills (c), \met{} is the only method to learn (all other methods are flat lines). All results are on the Stacking task. \label{fig:ablation_infer_and_temporal_correlation}}
\end{figure}


\subsubsection{Utility of Flexible Temporal Abstraction}
\label{sec:temporal_abstraction}

\paragraph{Temporally-correlated exploration}
Figs. \ref{fig:single-skill} and \ref{fig:multiple-skill} illustrate the importance of temporally-correlated exploration that arises from our formulation in Section \ref{method}. For this analysis we additionally run a version of our algorithm called `\met{} (without temporal abstraction)' where a new skill must be chosen at each timestep ($K=\{1\}$).
When given a single (near-)optimal skill\footnote{The near-optimal skill for the Stacking task places the green object on the yellow one without moving the gripper away.}, all methods including regularisation and fine-tuning perform similarly (Fig. \ref{fig:single-skill}). However,
when we use more than one sub-optimal skill, temporally correlated exploration is crucial for learning (Fig. \ref{fig:multiple-skill}).


\paragraph{Variable temporal abstraction}
Fig. \ref{fig:ablation_temporal_abstraction} analyses the importance of the flexible temporal abstraction of \met \
by comparing our method against a version dubbed `\met{} (fixed temporal abstraction \rebuttal{- X})' where each skill, once chosen, is held fixed for a given duration \rebuttal{of X timesteps} (\rebuttal{[10, 50, 100, 150, 200]} timesteps in a 600 step episode). We observe that \rebuttal{the optimal fixed skill length varies from task to task (see Fig. \ref{fig:fixed_skill_stack} vs \ref{fig:fixed_skill_pyramid}) and, most importantly,} the performance on harder tasks (especially triple-stacking) degrades when using this constraint. Thus, flexibly choosing the duration for each skill is quite important. 

\begin{figure}
\centering
\includegraphics[height=0.7cm, trim=0 0 0 0, clip=true]{assets/figures/fixed_skill_length_legend.png}

  \centering
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth,]{assets/figures/skill_length_stacking.png}
    \vspace{-1.5em}
    \caption{Stacking \label{fig:fixed_skill_stack}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth,]{assets/figures/skill_length_pyramid.png}
    \vspace{-1.5em}
    \caption{Pyramid Stacking\label{fig:fixed_skill_pyramid}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth,]{assets/figures/skill_length_triple.png}
    \vspace{-1.5em}
    \caption{Triple stacking}
  \end{subfigure}
\vspace{-0.5em}
\caption{The variable temporal abstraction of \met{} is especially crucial for learning harder tasks. \label{fig:ablation_temporal_abstraction}}
\end{figure}





==> S&T_arxiv2/iclr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> S&T_arxiv2/intro.tex <==
\section{Introduction}

The ability to effectively build on previous knowledge, and efficiently adapt to new tasks or conditions, remains a crucial problem in Reinforcement Learning (RL). %
It is particularly important in domains like robotics where data collection is expensive and where we often expend considerable human effort designing reward functions that allow for efficient learning.

Transferring previously learned behaviors as skills can decrease learning time through better exploration and credit assignment, and enables the use of easier-to-design (e.g. sparse) rewards.
As a result, skill transfer has developed into an area of active research, but existing methods remain limited in several ways. 
For instance, fine-tuning the parameters of a policy representing an existing skill is conceptually simple. However, allowing the parameters to change freely can lead to a catastrophic degradation of the behavior early in learning, especially in settings with sparse rewards \citep{igl2020transient}.
An alternative class of approaches focuses on transfer via training objectives such as regularisation towards the previous skill. %
These approaches have been successful in various settings \citep{ross2011reduction, Galashov2019infoasym, Tirumala2020priorsjournal, rana2021bayesian}, but their performance is strongly dependent on hyperparameters such as the strength of regularisation. If the regularisation is too weak, the skills may not transfer. If it is too strong, %
learning may not be able to deviate from the transferred skill.
Finally, Hierarchical Reinforcement Learning (HRL) allows the composition of existing skills via a learned high-level controllers, sometimes at a coarser temporal abstraction \citep{sutton1999between}. Constraining the space of behaviors of the policy to that achievable with existing skills can dramatically improve exploration \citep{nachum2019does} but it can also lead to sub-optimal learning results if the skills or level of temporal abstraction are unsuitably chosen \citep{sutton1999between, wulfmeier2021data}. \rebuttal{As we will show later (see Section \ref{experiments}), these approaches demonstrably fail to learn in many transfer settings.}

Across all of these mechanisms for skill reuse we find a shared set of desiderata. %
In particular, an efficient method for skill transfer should 1) reuse skills and utilise them for exploration at coarser temporal abstraction, 2) not be constrained by the quality of these skills or the used temporal abstraction, 3) prevent early catastrophic forgetting of knowledge that could be useful later in learning.



With \method~(\met), we develop a method to satisfy these desiderata. We focus on the transfer of skills via their generated experience inspired by the Collect \& Infer perspective~\citep{riedmiller2022collect_infer, Riedmiller2018sacx}. Our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration via fast composition, but allows the final solution to deviate from the prior skills. 
More specifically the approach learns two separate components: First, we learn a high-level controller, which we refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, incentivizing it to rapidly collect task-relevant data. Second, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained off-policy with the same objective \rebuttal{and in parallel with the scheduler}. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand. \rebuttal{This addition improves over the common use of reloaded policies in hierarchical agents such as the options framework \citep{sutton1999between} and prevents the high-level controller from being constrained by the reloaded skills.}


The key contributions of this work are the following:  
\begin{itemize}
    \item We propose a method to 
    fulfil the desiderata for 
    using skills for knowledge transfer, and evaluate it on a range of \rebuttal{embodied settings in which we may have related skills and need to transfer in a data efficient manner.}
    \item We compare our approach to transfer via vanilla fine-tuning, hierarchical methods, and imitation-based methods like DAGGER and KL-regularisation. Our method consistently performs best across all tasks. 
    \item In additional ablations, we disentangle the importance of various components: temporal abstraction for exploration; distilling the final solution into the new skill; and other aspects.%
\end{itemize}




    
    
    
    
    
    
    
    
    
    















==> S&T_arxiv2/method2.tex <==
\section{Method}
\label{method}



The method we propose in this paper, named \textit{\method~(\met)} (Fig. \ref{fig:SkillS})
explicitly separates the data collection and task solution inference processes in order to better accommodate the requirements of each. The data collection is performed by the \textit{scheduler}, a high-level policy that chooses the best skills to maximize the task reward obtained from the environment. The task solution is learned via an off-policy learning algorithm that optimises a \textit{new skill} $\pi_{N}(a|s, \phi)$ for the given task.

By avoiding assumptions about the representation and source of the underlying skills, we can use these existing behaviors agnostic to how they were generated.
The agent has no access to any prior information on the quality of the skills and their relevance for the new task.  While most of our experiments in Section~\ref{experiments} focus on reusing skills that are useful for the task, we conduct a detailed ablation study that investigates the robustness with respect to the number and quality of skills used.

\begin{figure}
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/images/SkillS_newskill2.png}
    \caption{\label{fig:SkillS}}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{assets/images/action_and_counter_new3.png}
    \caption{\label{fig:action_and_counter}}
\end{subfigure}
\caption{\textbf{a) The \method{} framework.} Data is collected by the scheduler by sequencing selected skills among a set of pre-trained (frozen) skills and the new skill. This data is used to improve the scheduler using HCMPO (see Section \ref{hcmpo}) and the new skill via CRR. \textbf{b) Scheduler action and counter sampling.} At time $t=0$ the scheduler samples an action $z_0=[i_0; k_0]$ i.e. the skill with index $i_0$ is applied to the environment for $k_0$ time steps. When ($t=k_0$), the scheduler samples a new action, the counter is set to the new length $c_t=k_t$ and decreased every time step.}
\end{figure}

\subsection{Scheduler}
The scheduler is represented by a multivariate categorical policy $\pi_{S}(z = [i; k]|s, \theta)$ that outputs an action $z$ consisting of:
\begin{itemize}
    \item the index $i \in [0, .., N]$ of the skill to execute among the available skills $\bar{\mathrm{S}} = \mathrm{S} \cup \{\pi_{N}(a|s, \phi)\}$, where $\mathrm{S} = \{\pi_i(a|s)\}_{i=0}^{N-1}$ are the $N$ previously trained and frozen skills  
    and $\pi_{N}(a|s, \phi)$ is the new skill, and
    \item the number of steps the skill is executed for $k \in \mathrm{K}$ (the \textit{skill length}), where $\mathrm{K}$ is a set of available skill lengths (positive integers) with cardinality $|\mathrm{K}| = M$.
\end{itemize}

Whenever a new action $z = [i; k]$ is chosen by the scheduler, the skill $\pi_{i}(a|s)$ is executed in the environment for $k$ timesteps.
The scheduler does not sample any new action until the current skill length $k$ is expired (see Fig. \ref{fig:action_and_counter}). 
Choosing $k>1$ means that the scheduler selects a new skill at a coarser timescale than the environment timestep. This induces temporal correlations in the actions, which are important for successful skill-based exploration in sparse-reward tasks (see Section \ref{experiments}).

Choosing one skill for multiple timesteps affects the agent's future action distributions and therefore future states and rewards.
We add an auxiliary \textit{counter} variable $c$ to the observations to retain the Markov property. Whenever the scheduler chooses a new action $z = [i; k]$ the counter is set equal to the chosen skill duration $c = k$. It is then decreased at every time step ($c_{t+1} = c_t - 1$) until the chosen skill duration has been reached ($c=0$) and the scheduler chooses a new action (see Fig. \ref{fig:action_and_counter}). The counter is crucial for learning of the critic, as detailed in Section \ref{hcmpo}.


Data is collected in the form $(s_t, a_t, z_t, c_t, r_t, s_{t+1})$ and is used both to train the scheduler and the new skill. The scheduler is trained only using the high-level actions $( \mathbf{z_t}, c_t, r_t, s_{t+1})$
with the accumulated task return over the episode as objective (Eq. \ref{eq:rl}).

We introduce an off-policy algorithm, \textit{Hierarchical Categorical MPO} (HCMPO) to train the scheduler. While any RL algorithm could be used as a starting point,
HCMPO builds upon a variant of Maximum A-Posteriori Policy Optimisation (MPO)~\citep{abdolmaleki2018maximum} with a discrete action space~\citep{neunert2020continuous}.
More details are provided in Section \ref{hcmpo}.

\subsection{New Skill}
The new skill $\pi_{N}(a|s, \phi)$ interacts with the environment only when chosen by the scheduler. 
It is trained with the data only including the low-level action $(s_t, \mathbf{a_t}, r_t, s_{t+1})$ %
collected by the frozen skills $\mathrm{S}$ and the new skill itself according to the scheduler decisions. Given the strongly off-policy nature of this data\footnote{The new skill is initially rarely executed as 
it commonly 
provides lower rewards than reloaded skills.}, offline RL algorithms are most suited for learning the new skill. For this work, we use Critic Regularized Regression \citep{wang2020critic}.\footnote{We present an analysis of the advantages of using offline methods like CRR against off-policy methods like MPO in Appendix \ref{sec:appendix_mpo_v_crr}.}%

Note that, although the scheduler and the new skill are trained with the same objective of maximizing the task reward (Eq. \ref{eq:rl}), we consider the new skill to provide the final solution for the task at hand, as it can reach higher performance. Whereas the scheduler acts in the environment via prelearned skills \textit{fixed} to avoid degradation of the prior behaviors, the new skill is \textit{unconstrained} and can thus fully adapt to the task at hand. In Section \ref{separate_inference} we show how the scheduler and the new skill successfully tackle the two different problems of rapidly collecting task-relevant data (the scheduler) and slowly distilling the optimal task solution from the gathered experience (the new skill).


\subsection{Training the Scheduler} \label{hcmpo} 
In this section we derive the policy evaluation and improvement update rules of our proposed algorithm, Hierarchical Categorical MPO (HCMPO), used for training the scheduler.


\textbf{Policy Evaluation}
In order to derive the updates, we take into account the fact that if $k_{t}$ time steps have passed, i.e. the counter $c_{t}$ has expired, the scheduler chooses a new action $z_t=[i_t; k_t]$ at time $t$. It keeps the previous action  $z_t=z_{t-1}=[i_{t-1}; k_{t-1}]$ otherwise. %
\begin{equation}
  \label{policy_eval}
    Q(s_t, c_t, i_t, k_t) \xleftarrow{} r_t +  \gamma \begin{cases}
    E_{\pi_{S}(i;k|s_{t+1})}[Q(s_{t+1}, c_{t+1}, i, k, \theta)] \text{ if } c_{t+1}= 1 \\
    Q(s_{t+1}, c_{t+1} = c_t - 1, i_{t+1}  = i_t, k_{t+1} = k_t) \text{ otherwise.}\\
\end{cases}
\end{equation}
If the scheduler has chosen a new action in the state $s_{t+1}$, the critic in state $s_t$ is updated with the standard MPO policy evaluation, i.e. with the critic evaluated using actions sampled from the current scheduler policy in the next state $i, k \sim \pi_{S, \theta}(i;k|s_{t+1})$. In all the other states instead, the critic is updated with the critic computed using the action $z_{t+1}$ actually taken by the scheduler, which is $z_{t+1} =  z_t = [i_t; k_t]$. More details on the derivations of Eq. \ref{policy_eval} are available in Appendix \ref{appendix:policy_eval}.

\textbf{Policy Improvement}
The scheduler policy is improved via the following mechanism but only on transitions where a new action is sampled by the scheduler:
\begin{equation}
   \label{policy_impr}
    \pi_{S}^{n+1} = \arg \max_{\pi_{S}} \int  \int q(z|s) \log(\pi_{S}(z| s, \theta)dz ds \text{ with }
    q(z|s) \propto \pi_{S}^{n}(z|s) \exp\Big({Q^{\pi_{S}^{n}}(s, \mathbf{c = 1}, z)}\Big),
\end{equation}
where $n$ is the index for the learning updates.


\subsection{Data Augmentation}
Eq. \ref{policy_eval} and \ref{policy_impr} show that only a subset of the available data would be actively used for learning the scheduler, i.e. only those states $s$ where the scheduler chooses a new action $z = [i; k]$. This effect is even stronger if the skill lengths $k \in \mathrm{K}$ are $>> 1$, as a new scheduler action $z$ is sampled less frequently. While large skill lengths induce temporal correlations that are important for skill-based exploration, it has the side effect of decreasing the data actively contributing to improve the scheduler. In order to maximize sample efficiency without sacrificing exploration,
we duplicate trajectories with long skill executions by also considering the same skill being executed repetitively for shorter amount of time\footnote{For example, a trajectory of a skill executed for 100 timesteps could be generated equivalently by executing it once for 100 steps or 10 times consecutively for 10 steps each.}. More details regarding the augmentation are described in Appendix \ref{appendix:data_aug} and we include ablations in Appendix \ref{appendix:data_aug_ablation}.














==> S&T_arxiv2/related.tex <==
\section{Related Work}
The study of skills in RL is an active research topic that has been studied for some time \citep{thrun1994finding, bowling1998reusing, bernstein1999reusing, pickett2002policyblocks}. A `skill' in this context refers to any mapping from states to actions that could aid in the learning of new tasks. These could be pre-defined motor primitives \citep{Schaal2005primitive, mulling2013learning, ijspeert2013dynamical, Paraschos2013primitives, lioutikov2015probabilistic, paraschos2018using}, temporally-correlated behaviors inferred from data \citep{niekum2011clustering, ranchod2015nonparametric, kruger2016efficient, lioutikov2017learning, shiarlis2018taco, kipf2019compile, Merel2019npmp, shankar2019discovering,tanneberg2021skid} or policies learnt in a multi-task setting \citep{heess2016learning, Hausman2018latentspace, Riedmiller2018sacx}. It is important to note that our focus in this work is not on learning skills but instead on how to to best leverage a given set of skills for transfer. 

Broadly speaking, we can categorise the landscape of transferring knowledge in RL via skills into a set of classes (as illustrated in Fig. \ref{fig:transfer_mechanisms}): direct reuse of parameters such as via fine-tuning existing policies \citep{rusu2015policy, parisotto2015actor, Schmitt2018KickstartingDR}, 
direct use in Hierarchical RL (HRL) where a high-level controller is tasked to combine primitive skills or options \citep{sutton1999between, heess2016learning, bacon2017option,wulfmeier2019compositional, daniel2012hierarchical,peng2019mcp},
transfer via the training objective such as regularisation towards expert behavior \citep{ross2011reduction, Galashov2019infoasym, Tirumala2020priorsjournal} and transfer via the data generated by executing skills \citep{Riedmiller2018sacx,Campos2021BeyondFT,torrey2007relational}.

\textbf{Fine-tuning} often underperforms because neural network policies often do not easily move away from previously learned solutions \citep{ash2020warm, igl2020transient, Nikishin2022ThePB} and hence may not easily adapt to new settings. As a result some work has focused on using previous solutions to `kickstart' learning and improve on sub-optimal experts \citep{Schmitt2018KickstartingDR, jeong2020learning, abdolmaleki2021multi}. When given multiple skills, fine-tuning can be achieved by reloading of parameters via a mixture \citep{daniel2012hierarchical, wulfmeier2019compositional} or product \citep{peng2019mcp} policy potentially with extra components to be learnt.

An alternative family of approaches uses the skill as a `behavior prior' to to generate \textbf{auxiliary objectives} to regularize learning \citep{liu2021from}. This family of approaches have widely and successfully been applied in the offline or batch-RL setting to constrain learning \citep{jaques2019way, wu2019behavior, siegel2020keep, wang2020critic, peng2020advantage}. When used for transfer learning though, the prior can often be too constraining and lead to sub-optimal solutions \citep{rana2021bayesian}.

Arguably the most widely considered use case for the reuse of skills falls under the umbrella of \textbf{hierarchical} RL. These approaches consider a policy that consists of two or more hierarchical `levels' where a higher level controllers modulates a number of lower level skills via a latent variable or goal. This latent space can be continuous \citep{heess2016learning, Merel2019npmp, Hausman2018latentspace, Haarnoja2018lsp, Lynch2019play, Tirumala2019priors, pertsch2020accelerating, Ajay2021opal, Singh2021parrot, bohez2022imitate}, discrete \citep{florensa2017stochastic, Wulfmeier2020rhpo, seyde2022strength} or a combination of the two \citep{Rao2021LearningTM}. 

A major motivation of such hierarchical approaches is the ability for different levels to operate at different timescales which, it is argued, could improve exploration and ease credit assignment. The most general application of this, is the Options framework \citep{sutton1999between, bacon2017option, wulfmeier2021data} that operates using temporally-extended options. This allows skills to operate at longer timescales that may be fixed \citep{li2019sub,zhang2020hierarchical, Ajay2021opal} or with different durations \citep{bacon2017option, wulfmeier2021data,Salter2022MO2MO}. The advantage of modeling such temporal correlations has been attributed to benefits of more effective exploration \citep{nachum2019does}. However, constraining the policy in such a way can often be detrimental to final performance \citep{bowling1998reusing, jong2008utility}. 

Compared to other hierarchical methods such as the options framework, our method uses a final unconstrained, non-hierarchical solution and learn temporal abstraction as a task-specific instead of skill-specific property. %
In this way, we benefit from temporally correlated exploration without compromising on final asymptotic performance by distilling the final solution.
Our work is closely related to \textbf{transfer via data} for off-policy multi-task RL as explored by \citep{Riedmiller2018sacx, hafner2020towards} and initial work in transfer learning \citep{Campos2021BeyondFT,torrey2007relational}. 
We extend these ideas to the compositional transfer of skills.%

\begin{figure}[t]
\centering
\includegraphics[scale=0.2]{assets/images/transfer_mechanisms3.png}
\caption{Transfer mechanisms for skills: Direct use via 1. fine-tuning or 2. hierarchical policies, 3. auxiliary training objectives, 4. exploration and data generation. Grey and green respectively denote new policy components and transferred skills.}
\label{fig:transfer_mechanisms}
\end{figure}








==> S&T_arxiv2/title.tex <==


\title{SkillS: Adaptive Skill Sequencing for \\Efficient Temporally-Extended Exploration}



==> backup/experiments.tex <==
\section{Experiments}
\label{experiments}

\subsection{Setup}
\label{experiments:setup}

The domains we consider for our experimental analysis can be broadly split into two categories: `Manipulation' and `Locomotion'. 

In the `Manipulation'  setting (see Figure \ref{fig:domains} (left)), a Sawyer robot arm equipped with Robotiq gripper
(for details on the setup, see Appendix \ref{appendix:skills}) is rewarded for bringing a set of three objects (green, yellow and blue) into a particular configuration. The configurations we consider include (in increasing order of complexity): `Lift' (lift the green object), `Stack' (stack green on yellow), `Pyramid` (stack green as a bridge on yellow and blue) and `Triple stack` (stack green on yellow and yellow on blue). As the task gets harder, we leverage previous task solutions as skills for the new setting. This is a natural transfer setting to test an agent's ability to build on previous knowledge and solve increasingly complex tasks. 
% For example, `Stack'  has access to the `Lift' skills while `Pyramid' has access to `Lift' and `Stack' skills.
For a full list of skills and tasks considered see Appendix \ref{appendix:experiment_details}).

For `Locomotion' (see Figure \ref{fig:domains} (right)), we consider a task where a bipedal OP3 robot \citep{} receives a sparse reward for scoring a goal with a wall blocking part of the path. Unlike in `Manipulation' where the transfer task changes, here we consider transferring to the same task but with different environment dynamics; a common problem faced when operating in the real world.

All the transfer tasks we consider use sparse rewards which are easier to define and are practically relevant for domains like robotics. We consider an off-policy distributed learning setup with a single actor and experience replay with full details provided in Appendix \ref{appendix:training_details}.

\begin{figure}
  \centering
    \includegraphics[width=\textwidth]{assets/images/domains.png}
\caption{\textbf{Domains:} The experimental domains used: (from left to right) `Manipulation' - Lift, Stack, Pyramid, Triple Stack and `Locomotion'- Goal-scoring. \label{fig:domains}}
\end{figure}

\subsection{How we analyse the performance}
Our method \met{} consists of two learning processes, one designed to quickly collect useful data (the scheduler) and one to distill the best solution for the task from the same data (the new skill). As our primary interest is in the task solution, unless otherwise specified, we report the \textit{performance of the new skill} when executed in isolation on the environment for the entire episode (see Fig. \ref{fig:skill_analysis}).
% The performance of the data collection could be instead analysed by looking at the reward collected by the Skill Scheduler itself (Fig. \ref{fig:scheduler_analysis}), see the Appendix for this further analysis. \giulia{Shall we keep it or not?} 
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.275\textwidth}
    \centering
  \includegraphics[width=\textwidth]{assets/images/new_skill_analysis_3.png}
  \vspace{1pt}
  \caption{\label{fig:skill_analysis}}
  \end{subfigure}
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
  \includegraphics[width=\textwidth]{assets/images/scheduler_analysis_2.png}
  \vspace{0.5pt}
   \caption{\label{fig:scheduler_analysis}}
  \end{subfigure}
     \hspace{4pt}
  \begin{subfigure}[b]{0.36\textwidth}
  \includegraphics[height=0.95cm, width=0.98\linewidth, trim=0 0 0 0, clip=true]{assets/figures/skill_execution_legend.png}
\includegraphics[width=\linewidth]{assets/figures/skill_execution.png}
\caption{\label{fig:skill_execution_plot}}
\end{subfigure}
\caption{\textbf{a) - b) Performance analysis} The new skill is evaluated by executing it in the environment for the entire episode (\ref{fig:skill_analysis}). This differs from the way the data is collected, as at training time the new skill can interact with the environment time only when selected by the scheduler (\ref{fig:scheduler_analysis}). \textbf{c) Skill execution:} The plot shows the consecutive execution of each skill, i.e. the number of timesteps each skill has been consecutively executed for. \giulia{replace plot}}
\end{figure}

\giulia{To update with total execution}
Before focusing on the new skill performance in the next sections, it is worth showing how the scheduler chooses the skills to interact with the environment.
In Fig. \ref{fig:skill_execution_plot} we show the skill selection during the training by plotting the average \textit{consecutive} execution for each skill. We assume 7 skills are available, some of them needed for solving the task at hand (`reach green', `close fingers'), while the others act as a distractor (e.g. `reach yellow' or `open fingers'). At the beginning the scheduler quickly selects the most useful skills (`reach green', `close fingers') while discarding those less relevant to the task (look at the drop in executing `reach yellow' or `reach blue'). Also, the scheduler does not initially choose the new skill as it performs poorly at the beginning of the training. Once the new skill improves (after roughly 200- episodes), the scheduler quickly understands to select it more often, becoming eventually the most executed skill.


\subsection{Analysis: Sparse locomotion and manipulation}
The goal of this section is to analyse how the different skill reuse methods perform when transferring to the domains defined in Section \ref{experiments:setup}. Figure \ref{fig:manipulation_sparse} shows the performance of skill-based approaches on the `Manipulation' domains \footnote{Given the sparse nature of the reward, note that most methods fail to learn at all and show up as flat lines in the plot.}. We observe that among all the methods that we considered only \met \ can learn effectively in these domains even though other methods have access to the same set of skills. Importantly this illustrates that reusing skills on its own is insufficient to guarantee good transfer performance. 

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{assets/figures/manipulation_sparse.png}
%   \caption{\textbf{Sparse Manipulation:} Performance of various skill transfer mechanisms on sparse manipulation tasks.}
%   \label{fig:manipulation_sparse}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sparse.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_sparse.png}
    \caption{Lifting}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sparse.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_sparse.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_sparse.png}
    \caption{Triple Stacking}
  \end{subfigure}
\caption{Performance of various skill transfer mechanisms on sparse-reward manipulation tasks. For each task, all approaches are given the previous, easier skills (see Appendix for details) to learn the new task.}
\label{fig:manipulation_sparse}
\end{figure}

TODO(dhruvat): Insert OP3 results here once ready.
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/op3_legend_goal_scoring.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/op3_goal_scoring.png}
  \end{subfigure}
\caption{Performance on sparse-reward locomotion task.}
\label{fig:op3_goal_scoring}
\end{figure}


\subsection{Ablations}
In this section we analyse \met \ to test its robustness and tease apart which of it's components are important and under what conditions. The key questions we seek to answer through our analysis are:
\begin{enumerate}
    \item How robust is \met \ to the number and quality of skills used?
    \item How does the analysis change when investing engineering effort to design dense rewards?
    \item Are there advantages to the flexibility of the infer mechanism? \dhruva{This feels a bit out of place here. Figure out structure once OP3 results are in.}
    \item Is the flexible temporal abstraction useful?
    \item How important is the temporally correlated exploration mechanism of \met?
    \item Does the separate inference mechanism provide any advantage?
    \giulia{Maybe point 2. and 6. can be merged together and we can analyse everything together?}
\end{enumerate}

\subsubsection{Robustness to number and type of skills}

Figure \ref{fig:ablation_num_skills} evaluates \met \ on the Stacking, Pyramid and Triple-stacking domains while changing the skill set $S$. For this analysis we vary the number of skills and the types of skills that the method has access to. In particular, we include a varying number of `distractor' skills that are not directly relevant for the task (e.g. reach `blue' for a task where `red' needs to be stacked, details in the Table \ref{tab:skills} in Appendix \ref{appendix:skills}). For the easier tasks of Stacking and Pyramid, the method is quite robust to various kinds of skills as long as there are \textit{some useful} skills in the set. When given only distractor skills, \met \ understandably fails to learn anything. On the most challenging task of Triple-stacking, increasing the number of skills has a detrimental effect of performance. We hypothesize that since more skills can greatly increase the size of the search space, it becomes much harder to randomly stumble onto the task solution. \dhruva{We could add a forward reference to the Discussion section here and discuss there ways to improve the method in future work to try to address this.}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{assets/figures/ablation_num_skills.png}
%   \caption{\textbf{Robustness to skills:} Performance when the number and type of skills changes.}
%   \label{fig:ablation_num_skills}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.5cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_skill_num.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_skill_num.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_skill_num.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stacking_skill_num.png}
    \caption{Triple Stacking}
  \end{subfigure}
\caption{\textbf{Robustness to skills:} Performance when the number and type of skills changes.}
\label{fig:ablation_num_skills}
\end{figure}

\subsubsection{Performance with dense rewards.}

Figure \ref{fig:manipulation_staged} shows the performance with all skill transfer methods on the `Lift' and `Stacking' tasks when the agent has access to dense rewards. We observe that, in contrast to the sparse reward results of Figure \ref{fig:manipulation_sparse}, all methods learn effectively when provided with dense rewards. Since the reward provides a useful and reliable signal to guide learning there is less need to generate good exploration data using previous skills. The advantage of skill-based methods is thus primarily in domains where defining a dense reward is challenging but the required sub-behaviors are easier to specify.

% \begin{figure}
%   \centering
%   \includegraphics[width=\textwidth]{assets/figures/manipulation_staged.png}
%   \caption{\textbf{Dense Manipulation:} Performance on dense manipulation tasks.}
%   \label{fig:manipulation_staged}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_dense.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_dense.png}
    \caption{Lifting}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_dense.png}
    \caption{Stacking}
  \end{subfigure}
\caption{Performance on dense-reward manipulation tasks. With carefully-tuned shaped rewards on simpler tasks, skill reuse is not as beneficial and all methods can learn effectively.}
\label{fig:manipulation_staged}
\end{figure}

\subsubsection{Flexibility of collect and infer}

% \begin{figure}
%   \centering
%   \includegraphics[height=6cm]{assets/figures/flexibility_c_i.png}
%   \caption{\textbf{Flexibility of collect and infer}}
%   \label{fig:ablation_separate_infer}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_flexibility.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{assets/figures/blocks_lift_flexibility.png}
    \caption{Lifting}
    \label{fig:blocks_lift_flexibility}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_flexibility.png}
    \caption{Stacking}
    \label{fig:ablation_separate_infer}
  \end{subfigure}
\caption{Performance of \met~when combined with other approaches to transfer, showing its flexibility.}
\label{fig:manipulation_flexibility}
\end{figure}

\subsubsection{Flexible temporal abstraction}

Figure \ref{fig:ablation_temporal_abstraction} analyses the importance of the flexible temporal abstraction of \met. For this, we compare our method against a version dubbed `\met{} (fixed temporal abstraction)' where each skill, once chosen, is held fixed for a given duration (200 timesteps for episode of 600 timesteps). We observe that the performance on harder tasks (especially triple-stacking) degrades when using this constraint. Thus, the ability to flexibly choose the duration for which the skill is applied is quite important. \dhruva{We could make a point about options here and in the next ablation.}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.7\textwidth]{assets/figures/ablation_temporal_abstraction.png}
%   \caption{\textbf{Temporal abstraction:} Importance of flexible temporal abstraction.}
%   \label{fig:ablation_temporal_abstraction}
% \end{figure}
\begin{figure}
\begin{center}
\includegraphics[height=0.5cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_flex_abs.png}
\end{center}
  \centering
  \begin{subfigure}[b]{0.31\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_flex_abs.png}
    \caption{Stacking}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_pyramid_flex_abs.png}
    \caption{Pyramid}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_triple_stack_flex_abs.png}
    \caption{Triple stacking}
  \end{subfigure}
\caption{\textbf{Temporal abstraction:} Importance of flexible temporal abstraction.}
\label{fig:ablation_temporal_abstraction}
\end{figure}

\subsubsection{Temporally correlated exploration}

Figure \ref{fig:ablation_temporal_correlation} illustrates the importance of temporally correlated exploration that arises from our formulation in Section \ref{method}. For this analysis we additionally run a version of our algorithm called `\met{} (without temporal abstraction)' where a new skill must be chosen at each timestep instead (i.e. $K=\{1\}$). In Figure \ref{fig:ablation_temporal_correlation} (left) we observe that, when given a single (near-)optimal skill\footnote{The near-optimal skill places the green object on the yellow one without moving the gripper away.}, all methods including regularisation and fine-tuning perform similarly. However, as shown in Figure \ref{fig:ablation_temporal_correlation} (right), when we use more than one sub-optimal skills temporally correlated exploration is crucial for learning.
 
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{assets/figures/ablation_temporal_correlation.png}
%   \caption{\textbf{Temporal correlation:} Importance of temporally correlated exploration.}
%   \label{fig:ablation_temporal_correlation}
% \end{figure}
\begin{figure}
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
  \includegraphics[height=0.75cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_temporal2.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_single_temporal.png}
    \caption{Single optimal skill}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\linewidth]{assets/figures/blocks_multi_temporal.png}
    \caption{Multiple sub-optimal skills \label{fig:ablation_temporal_correlation}}
  \end{subfigure}
    \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[height=1cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sep_infer.png}
    \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sep_infer.png}
    \caption{\label{fig:ablation_separate_infer}}
    \end{subfigure}
\caption{\textbf{a) - b) Temporal correlation:} Importance of temporally correlated exploration. \textbf{c) Separate infer:} Importance of having separate inference mechanism.}
\end{figure}

\subsubsection{Separate `infer' mechanism}
\label{separate_inference}

Finally, we conduct an experiment to study the importance of a separate `inference' (learning) mechanism as prescribed by the `Collect and Infer` paradigm. Figure \ref{fig:ablation_separate_infer}
compares the performance of \met{} (i.e. the inferred new skill when executed alone, as shown in Figure \ref{fig:skill_analysis}) against the performance of: `Scheduler' i.e. the Scheduler when executing the pre-trained skills $\mathrm{S}$ and the new skill (Figure \ref{fig:scheduler_analysis}), and `Scheduler (no new skill)', the performance of a Scheduler that can only execute the pre-trained fixed skills $\mathrm{S}$. As the figure shows, having a separate offline learning process is crucial for learning as the new skill (blue) outperforms the skill scheduler in performance, even when it can execute the new skill itself (light blue). The gap in performance is even more evident if the scheduler cannot access to the new skill (red).

% \begin{figure}
%   \centering
%   \includegraphics[height=6cm]{assets/figures/ablation_separate_infer.png}
%   \caption{\textbf{Separate infer:} Importance of having separate inference mechanism.}
%   \label{fig:ablation_separate_infer}
% \end{figure}
% \begin{figure}
% \begin{subfigure}[b]{0.5\textwidth}
% \includegraphics[height=1cm, trim=0 0 0 0, clip=true]{assets/figures/blocks_legend_sep_infer.png}
% \includegraphics[width=\linewidth]{assets/figures/blocks_stack_sep_infer.png}
% \caption{\textbf{Separate infer:} Importance of having separate inference mechanism.\label{fig:ablation_separate_infer}}
% \end{subfigure}
% \end{figure}

% What are our questions?
% \begin{itemize}
%     % \item Why is the scheduler so good? :) (placeholder)
%     \item How do different mechanisms for transfer relate to changes between source and target task? (what works well for dynamics vs reward changes)
%     \item How do different mechanisms for transfer relate to different task properties? (sparse v dense rewards)
%     \item How does temporal abstraction affect the performance for transfer?
%     \item How relevant is the distillation of behaviour into a single new policy? (and what makes it relevant)
% \end{itemize}

% The \met{} framework consists of two different learning processes with separate goals: 1) collecting data efficiently (the \method) and  2) inferring a task solution (the New Skill) that need to be evaluated separately.

% The way we evaluate the \method() and the New Policy is shown in Fig. \ref{fig:perf_eval}.
% \begin{itemize}
%     \item The \method{} is evaluated when executing the previously frozen skills and the New Policy. The desired behaviour consists of quickly collecting reward initially, while sub-optimal  performance at convergence are accepted\footnote{Sub-optimal performance at convergence is not a surprise as the \method does not have the same fine control as the New Policy, acting only at a larger time scale.}.
%     \item The New Policy is evaluated in isolation: it is executed for the entire episode. In this case, we want the final converged performance to be optimal as the New Policy is meant to provide the solution for the task.
% \end{itemize}

% In the next sections, we first analyse how the \method{} optimises the skill executions (Section \ref{skill_scheduler_analysis}) and then we analyse the quality of task solution we can obtain with the New Policy (Sections \ref{add section names}).
% \subsection{Skill scheduler vs baselines}

% \textit{How does our proposed method perform with respect to our transfer methods across different transfer scenarios (staged vs sparse reward), task changes vs dynamic changes?}

% \paragraph{Baselines}
% \begin{enumerate}
%     \item KL-reg
%     \item Skills reloading in RHPO
%     \item Fine-tuning (for OP3)
%     \item Dagger (Imitation learning)?
% \end{enumerate}

% \paragraph{Results}
% \begin{enumerate}
%     \item \textit{Sparse reward}. Skill scheduler outperforms all baselines
%     \begin{enumerate}
%     \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%             \item Stacking -> Pyramid
%             \item Stacking -> Triple stacking
%         \end{enumerate}
%      \item OP3 (transfer across dynamics or tasks?)
%         \begin{enumerate}
%             \item omni-directional walking -> 1v1?
%             \dhruva{Fine-tuning for omni-directional walking seems to fail even though reward is dense. We need to think about how to phrase this.}
%         \end{enumerate}
%     \end{enumerate}
% \end{enumerate}


% \begin{figure}
% \begin{center}
% \includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/images/blocks_legend_sparse.png}
% \end{center}
%   \centering
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{assets/images/blocks_lift_sparse.png}
%     \caption{Lifting}
%     \label{fig:blocks_lift_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_stack_sparse.png}
%     \caption{Stacking}
%     \label{fig:blocks_stack_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_pyramid_sparse.png}
%     \caption{Pyramid}
%     \label{fig:blocks_pyramid_sparse}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.22\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_triple_stacking_sparse.png}
%     \caption{Triple Stacking}
%     \label{fig:blocks_triple_sparse}
%   \end{subfigure}
% \caption{Transfer performance on four different manipulation tasks. For each task, all approaches are given the previous, easier skills (see Appendix for details) to learn the new task.}
% \end{figure}


% \subsection{Flexibility of separate Collect and Infer}
% \textit{Collect and infer gives great flexibility. What can we gain from it (i.e. using different methods for distilling the solution of the task)?}
% \subsubsection{Variations}
% \begin{enumerate}
%     \item Skill Scheduler vs
%     \item Skill Scheduler with KL-reg
%     \item Skill Scheduler with skills reloading in RHPO
% \end{enumerate}

% \subsubsection{Experiments}
% Maybe only with sparse reward here?
% \begin{enumerate}
%     \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%             \item Stacking -> Pyramid
%             \item Stacking -> Triple stacking
%             \dhruva{Perhaps here it is enough to include the hardest tasks?}
%         \end{enumerate}
%      \item OP3 (transfer across dynamics or tasks?)
%         \begin{enumerate}
%             \item omni-directional walking -> 1v1
%         \end{enumerate}
%     \end{enumerate}

% \subsection{Ablations on the Scheduler}
% \subsubsection{Dense versus sparse reward}
%  We show it is not so important with dense reward, everything works.
%     \begin{enumerate}
%         \item Blocks (transfer across tasks)
%         \begin{enumerate}
%             \item Reach -> Lift
%             \item Lift -> Stacking
%         \end{enumerate}
%         \item OP3 (transfer across dynamics)
%         \begin{enumerate}
%             \item walk -> walk
%         \end{enumerate}
%     \end{enumerate}
    
%     \begin{figure}
% \begin{center}
% \includegraphics[height=0.6cm, trim=0 0 0 0, clip=true]{assets/images/blocks_legend_sparse.png}
% \end{center}
%   \centering
%   \begin{subfigure}[b]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{assets/images/blocks_lift_dense.png}
%     \caption{Lifting}
%     \label{fig:blocks_lift_dense}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{0.45\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{assets/images/blocks_stack_dense.png}
%     \caption{Stacking}
%     \label{fig:blocks_stack_dense}
%   \end{subfigure}
% \caption{Transfer performance on manipulation tasks with dense rewards. With carefully tuned, shaped rewards, skill reuse is not as beneficial and all methods can learn effectively.}
% \end{figure}

% \subsubsection{Impact of different number of skills}
% \textit{What is the impact of different number and quality of skills on our method?}
% Only in ablations add all transfer settings (i.e. different number of skills).

% \subsubsection{Importance of temporal correlated exploration}
% \textit{How important is temporally correlated exploration?}

% \subsubsection{Comparison}
% \begin{itemize}
%     \item Skill Scheduler vs
%     \item Skill Scheduler with learned skill length=1
% \end{itemize}

% \subsubsection{Tasks}
% \begin{itemize}
%     \item Stacking (multiple skills and single skill)
% \end{itemize}

% \subsubsection{Importance of temporal abstraction and flexible skill length}
% \textit{How important is temporal abstraction and flexible skill length?}
% \subsubsection{Comparison}
% \begin{itemize}
%     \item Skill Scheduler with fixed skill length (200)
%     \item Skill Scheduler with learned skill length (v/s Q-scheduler?)
% \end{itemize}

% \subsubsection{Tasks}
% \begin{itemize}
%     \item Stacking
%     \item Pyramid (we need at least until pyramid to see the real benefits)
%     \item Triple stacking?
% \end{itemize}


% \subsubsection{Importance of separate Infer process}
% \textit{What are the benefits of distilling the solution in a separate learning process?}

% We could compare New policy distilled with skill scheduler with modular RHPO with frozen skills or the skill scheduler without the new policy?

% Big plus 1, here we should also discuss the connection to the options framework \citep{sutton1999between} - describing the scheduled version as essentially a reparametrised version of options

==> backup/intro_paragraph.tex <==
With \method~(\met), we develop a method to satisfy these desiderata. We focus on the transfer of skills via their generated experience inspired by the Collect \& Infer perspective~\citep{riedmiller2022collect_infer, Riedmiller2018sacx}. Our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration via fast composition, but allows the final solution to deviate from the prior skills. 
% ### MERGE
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained off-policy with the same objective. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.
% This can also be interpreted via the lens of fast and slow learning: the scheduler can quickly learn to compose existing temporally-abstract skills and reach a coarse solution, while the new policy can more slowly infer an optimal solution from the gathered data.
With these components, the desiderata are split into easier-to-solve subgroups.
% ### MERGE


Current versions/parts:

Nicolas
With \method~(\met), we develop a method to satisfy these desiderata. Inspired by the Collect \& Infer paradigm~\citep{riedmiller2022collect_infer},our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration and fast adaptation, but allows the final solution to deviate from the prior skills.
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we also refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, thus incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained via off-policy RL also to maximize the task reward. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.

Dushyant
... our approach takes advantage of hierarchical architectures with pretrained skills to achieve effective exploration, but allows the final solution to deviate from the prior skills.
This can also be interpreted via the lens of fast and slow learning: the scheduler can quickly learn to compose existing temporally-abstract skills and reach a coarse solution, while the new policy can more slowly infer an optimal solution from the gathered data.

Giulia
More specifically the approach learns two separate components: Firstly, we learn a high-level controller, which we also refer to as scheduler, which learns to sequence existing skills, choosing which skill to execute and for how long. The prelearned skills and their temporally extended execution lead to effective exploration. The scheduler is further trained to maximize task reward, thus incentivizing it to rapidly collect task-relevant data. Secondly, we distill a new policy, or skill, directly from the experience gathered by the scheduler. This policy is trained via off-policy RL also to maximize the task reward. Whereas the pretrained skills in the scheduler are fixed to avoid degradation of the prior behaviors, the new skill is unconstrained and can thus fully adapt to the task at hand.


==> backup/method.tex <==
\section{Method}
\label{method}
% - The method{} we propose reuses skills -> skill assumptions
% - The method{} we propose is based on Collect and Infer
% - High level description of all the pieces
% - Scheduler and HCMPO
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{assets/images/SkillS_newskill.png}
    \caption{\textbf{The \met{} framework.} The data collection is performed by the Scheduler, a high level policy that chooses the best skills to execute among a set of pre-trained and frozen skills and the New Skill. The data collected via the interaction of all the skills and the environment is used to improve the Scheduler and the New Skill in two learning processes, using respectively the algorithms Hierarchical Categorical MPO (see Section \ref{hcmpo}) and Critic Regulatirized Regression (CRR, \cite{wang2020critic}.}
    \label{fig:SkillS}
\end{figure}

% The method we propose in this paper, named \textit{\met}, exploits a set $\mathrm{S}$ of $N$ previously trained skills
% \begin{equation}
%     \mathrm{S} = \{\pi_i(a|s)\}_{i=0}^{N-1}
% \end{equation}
% to bootstrap data collection for learning challenging sparse reward tasks.

The method we propose in this paper, named \textit{\met}, is based on the Collect and Infer framework, which assumes that data collection and inference of the solution are carried out in two separate processes (Fig. \ref{fig:SkillS}). The data collection is performed by the \textit{Scheduler}, a high level policy that chooses the best skills to execute in the environment in order to gather interaction data. The inference process consists of an off-policy learning algorithm that optimizes a \textit{New Skill} $\pi_{N}(a|s, \phi)$ for the task at hand.%In particular our method consists of the \textit{\method{}} or \textit{Collector} that collects data using a set of  skills $\mathrm{S}$ and a \textit{New Skill} $\pi_{N, \phi}(a|s)$ that infers the task solution from this data.



\subsection{Scheduler}
The \textit{Scheduler} is represented by a categorical policy
\begin{equation}
    \pi_{S}(z = [i; k]|s, \theta)
\end{equation} that outputs an action $z$ consisting of:
\begin{itemize}
    \item the index $i \in [0, .., N]$ of the skill to execute among $N$ previously trained and frozen skills $\mathrm{S}$:
    \begin{equation}
        \mathrm{S} = \{\pi_i(a|s)\}_{i=0}^{N-1}  \text{ where } |\bar{\mathrm{S}}|= N,
    \end{equation}
    and the \textit{New Skill}:
    \begin{equation}
        \bar{\mathrm{S}} = \mathrm{S} \cup \{\pi_{N}(a|s, \phi)\} \text{ where } |\bar{\mathrm{S}}|= N + 1,
    \end{equation}
        \item and the number of steps the skill is executed for $k \in \mathrm{K}$ (the \textit{skill length}), where $\mathrm{K}$ is a set of available skill lengths (positive integers) with cardinality $|\mathrm{K}| = M$.
\end{itemize}

Whenever a new action $z = [i; k]$ is chosen by the \method{}, the skill $\pi_{i}(a|s)$ (or $\pi_{N}(a|s, \phi)$ if $i=N$) is executed in the environment for $k$ time steps.
The scheduler does not sample any new action until the current skill length $k$ is expired (see Fig. \ref{fig:action_and_counter}). %If none of the available skill lengths $k \in \mathrm{K}$ is 1, this means the scheduler chooses a new skill at a larger time scale than the time scale at which the skills interact with the environment. 
Choosing $k>1$ means that the scheduler selects a new skill at a time scale that is different from the one at which the agent interacts with the environment. This induces temporal correlations in the agent's action choices which are important for skill-based exploration to be successful in sparse-reward tasks (see Section \ref{experiments}).
%This enforces a \textit{temporally correlated exploration} that is crucial for solving challenging sparse reward tasks, as shown in Section \ref{experiments}. 

Choosing the skill duration up-front introduces a nonstationarity in the agent's behavior. 
%In order to take into account for the flexible time scale during training 
To be able to frame the learning problem as an MDP we make use of an auxiliary variable $c$ named \textit{counter}. Whenever the scheduler chooses a new action $z = [i; k]$ the counter is set equal to chosen skill duration $c = k$. It is then decreased at every time step ($c_{t+1} = c_t - 1$) until the chosen skill duration has been reached and %skill length expires and 
the scheduler chooses a new action (see Fig. \ref{fig:action_and_counter}). The counter is crucial for learning of the critic, as is shown in Section \ref{hcmpo}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{assets/images/action_and_counter_new.png}
    \caption{\textbf{Scheduler action sampling and counter value generation.} This figure explains through an example how the \method{} interacts with the environment. At time $t=0$ the Scheduler samples an action $z_0=[i_0; k_0]$. This means that the low-level actions sampled from the same skill with index $i_0 \in \bar{\mathrm{S}}$ are applied  on the environment for $k_0$ time steps (e.g. $a_t \sim \pi_{i_0}(a|s_t)$ for $t=0, \dots, k_0 -1$, with $k_0 = 10$ in the figure). The scheduler does not sample any new action $z = [i; k]$ until the skill length $k_0$ has expired, i.e. when $t=k_0=10$. The counter is reset to be equal to the new chosen skill length $c_t = k_t$ every time a new scheduler action $z_t = [i_t; k_t]$ is sampled and is decreased every time step.}
    \label{fig:action_and_counter}
\end{figure}


The data collected by the \method{} is in the form $(s, a, z, c, r)$ and is used both to train the scheduler to improve the data collection and the New Skill to solve the task. In particular, the \method{} is trained only using the high-level actions, i.e. $(s, \mathbf{z}, c, r)$. While many objectives could be used to optimize the scheduler for data collection, in this work we decide to use the accumulated task return over the episode with duration $T$, $\sum_{t=0}^{T}\gamma^t r_t.$



We propose a novel algorithm to train the \method{} named \textit{Hierarchical Categorical MPO} (HCMPO) that takes into account the flexible time scale at which the scheduler chooses new actions. More details are provided in Section \ref{hcmpo}.

\subsection{The New Skill}
The New Skill $\pi_{N}(a|s, \phi)$ interacts with the environment only when chosen by the Skill Scheduler. It is trained with the data $(s, a, r)$\footnote{The New Skill is trained using the low-level actions $a$ as it is required to output actions compatible with the environment. Note also that the counter $c$ is not used for training the New Skill.} collected by the frozen skills $\mathrm{S}$ and the New Skill itself according to the scheduler decisions. Given the strongly off-policy nature of this data\footnote{At the beginning of the training the New Skill is not executed often as it is less likely to provide reward signal than the other skills.}, we train  the New Skill via Critic Regularized Regression \citep{wang2020critic} using  the accumulated task reward $\sum_{t=0}^{T}\gamma^t r_t$ as training objective, like for the Scheduler.

Note that, although the \method{} and the New Skill are trained with the same objective, we consider the New Skill to provide the final solution for the task at hand, as it can reach higher performance being distilled \textit{from scratch} on the collected data. The Scheduler is instead more suited to quickly collect data by design: having access to pre-trained skills facilitates exploration but can lead to sub-optimal performance in the limit as it constraints the final behaviour.



\subsection{Hierarchical Categorical MPO} \label{hcmpo} 
The framework we propose in this work differs from existing work~\citep{Heess2016locomotioncontroller,Wulfmeier2020rhpo} as 1) the high-level controller (the Scheduler) and the \textit{new} low-level controller (the New Skill)\footnote{The other skills $\mathrm{S}$ are kept frozen and not trained.} are trained in two separate learning processes and 2) the high-level controller is trained taking into account the flexible time scale at which the high-level actions are chosen~\citep{??}. In this section we explain the algorithm Hierarchical Categorical MPO (HCMPO) we use for training the high-level controller, i.e. the \method{}.

HCMPO builds on top of MPO with discrete action space ~\citep{neunert2020continuous} modifying the way the Policy Evaluation (PE) and Improvement (PI) are executed.

\textbf{Policy Evaluation (PE).}
In order to derive the PE updates we write down the probability that the scheduler chooses an action $z_t$ and the relative counter $c_t$:
\begin{align}
  \label{action_prob}
  \pi(z_t, c_t | s_t, z_{t-1}, c_{t-1}) &= \nonumber \\
  \pi(i_t, k_t, c_t | s_t, i_{t-1}, k_{t-1}, c_{t-1}) &=
  \begin{cases}
    \pi_{S}(z_t = [i_t; k_t]|s_t, \theta)\delta(k_t, c_t)  \text{ if } c_{t-1} = 1 \\
  \delta(i_t - i_{t-1})\delta(k_t - k_{t-1})\delta(c_t - (c_{t-1} - 1)) \text{ otherwise.}
  \end{cases}
\end{align}


This takes into account the fact that, if $k_{t}$ time steps have passed, i.e. the counter $c_{t}$ has expired, the scheduler chooses a new action $z_t=[i_t; k_t]$ at time $t$. It keeps the previous action  $z_t=z_{t-1}=[i_{t-1}; k_{t-1}]$ otherwise.

We can now use \eqref{action_prob} to derive the PE update rules:
\begin{equation}
  \label{policy_eval}
    Q(s_t, c_t, i_t, k_t)& \xleftarrow{} r_t +  \gamma \begin{cases}
    E_{\pi_{S}(i;k|s_{t+1})}[Q(s_{t+1}, c_{t+1}, i, k, \theta)] \text{ if } c_{t+1}= 1 \\
    Q(s_{t+1}, c_{t+1} = c_t - 1, i_{t+1}  = i_t, k_{t+1} = k_t) \text{ otherwise.}\\
\end{cases}
\end{equation}
If in the state $s_{t+1}$ the Scheduler has chosen a new action, the critic in state $s_t$ is updated with the standard MPO policy evaluation, i.e. with the critic evaluated using actions sampled from the current Scheduler policy in the next state $i, k \sim \pi_{S, \theta}(i;k|s_{t+1})$. In all the other states instead, the critic is updated with the critic computed using the action $z_{t+1}$ actually taken by the Scheduler, which is $z_{t+1} =  z_t = [i_t; k_t]$.

\textbf{Policy Improvement}
The Scheduler policy is improved following the MPO PI mechanism but only using the state-action pairs that correspond to a new action sampled by the Scheduler:
\begin{align}
   \label{policy_impr}
    \pi_{S}^{n+1} = \arg \max_{\pi_{S}} \sum_j  \sum_h q_{h,j} & \log(\pi_{S}(i_h, k_h | s_j, \theta))\\
    q_{h,j} = \frac{\exp{Q^{\pi_{S}^{n}}(s_j, c_j = 1, i, k)}}{ \sum_i{\exp{Q^{\pi_{S}^{n}}(s_j, c_j = 1, i, k)}}},
\end{align}
where $n$ is the index for the learning updates, $j$ and $h$  the indices that takes into account respectively the sampled states and actions.

\subsection{Data Augmentation}
Equations \eqref{policy_eval} and \eqref{policy_impr} show that only a subset of the available data $(s, z, c, r)$ is actively used for learning the scheduler critic and policy, i.e. only those states $s$ where the scheduler chooses a new action $z = [i; k]$. This effect is even stronger if the skill lengths $k \in \mathrm{K}$ are $>> 1$, as a new scheduler action $z$ is sampled less frequently. While large skill lengths induce temporal correlations that are important for skill-based exploration, it has the side effect of decreasing the data actively contributing to improve the scheduler. In order to maximize sample efficiency without sacrificing exploration, we augment the data as described in the appendix.%as follows.

\markus{Recommended split for the appendix part here. This also includes moving the corresponding figure.}

We define a \textit{skill trajectory} $\tau$ as the sequence of  $k^*$ time steps where the same skill with index $i^*$ is executed:
\begin{equation}
    \tau = \{(s_t, z_t=[i^*, k^*], c_t, r_t)\}_{t=t_0}^{t=t_0 + k^* - 1}
\end{equation}
and $k_{min}$ the smallest skill length available to the scheduler ($k_{min} \leq k $ for $k \in \mathrm{K}$ and $k_{min} \in \mathrm{K}$ ).

For every trajectory $\tau$ with skill length $k^*$ that can be written as multiple of the minimum skill length $k_{min}$ ($ mod(k_t, k_{min}) = 0$), we generate a new \textit{duplicated skill trajectory} $\bar{\tau}$ pretending it was generated by a scheduler choosing the same skill $i^*$ multiple times with the smallest available skill length $k_{min}$ (see Fig. \ref{fig:data_augmentation}).  This generates a new trajectory that is compatible with the data actually collected, as the skill $i^*$ is executed for $k^*$ consecutive time steps also in $\bar{\tau}$. However, the new trajectory has more samples that are actively used for improving the scheduler and the policy, as it pretends the scheduler made a decision in more states. Both $\tau$ and $\bar{\tau}$ are added to the replay and used for training the scheduler. Technical details on the data augmentation are provided in Appendix \ref{appendix:data_aug}.



\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{assets/images/data_augmentation.png}
    \caption{\textbf{Example of data augmentation.} Let's assume we have a trajectory $\tau$ where the skill with index $i^*$ is executed for $k^* = 60$ time steps. The duplicated trajectory $\bar{\tau}$ is generated by pretending the scheduler chose the same skill with index $i^*$ every $k_{min}$ time steps, equal to 10 in our example. This generates a new trajectory $\bar{\tau}$ compatible with the low-level actions $a_t$ and state $s_t$ actually collected during the interaction with the environment. }
    \label{fig:data_augmentation}
\end{figure}



\markus{To add: This perspective is highly related to efficiently learning high-level controllers over sets of options in the context of intra-option learning (using data throughout option execution to train the inter option policy) \citep{sutton1999between}.}
